Verification of Semantically-Enhanced Artifact Systems (Extended Version)

Artifact-Centric systems have emerged in the last years as a suitable framework to model business-relevant entities, by combining their static and dynamic aspects. In particular, the Guard-Stage-Milestone (GSM) approach has been recently proposed to model artifacts and their lifecycle in a declarative way. In this paper, we enhance GSM with a Semantic Layer, constituted by a full-fledged OWL 2 QL ontology linked to the artifact information models through mapping specifications. The ontology provides a conceptual view of the domain under study, and allows one to understand the evolution of the artifact system at a higher level of abstraction. In this setting, we present a technique to specify temporal properties expressed over the Semantic Layer, and verify them according to the evolution in the underlying GSM model. This technique has been implemented in a tool that exploits state-of-the-art ontology-based data access technologies to manipulate the temporal properties according to the ontology and the mappings, and that relies on the GSMC model checker for verification.

==> submitted/0-abstract.tex <==
\begin{abstract} 

  Artifact-Centric systems have emerged in the last years as a suitable framework to model business-relevant entities, by combining their static and dynamic aspects. In particular, the Guard-Stage-Milestone (GSM) approach has been recently proposed to model artifacts and their lifecycle in a declarative way. In this paper, we enhance GSM with a Semantic Layer, constituted by a full-fledged OWL 2 QL ontology linked to the artifact information models through mapping specifications. The ontology provides a conceptual view of the domain under study, and allows one to understand the evolution of the artifact system at a higher level of abstraction.  In this setting, we present a technique to specify temporal properties expressed over the Semantic Layer, and verify them according to the evolution in the underlying GSM model. This technique has been implemented in a tool that exploits state-of-the-art ontology-based data access technologies to manipulate the temporal properties according to the ontology and the mappings, and that relies on the GSMC model checker for verification.


\end{abstract}


\endinput


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> submitted/1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

In the last decade, the marriage between processes and data has been
increasingly advocated as a key objective towards a comprehensive modeling and
management of complex enterprises \cite{CaDM13}. This requires to go beyond
classical (business) process specification languages, which largely leave the
connection between the process dimension and the data dimension underspecified,
and to consider data and processes as ``two sides of the same coin''
\cite{Reic12}.  In this respect, artifact-centric systems \cite{NiCa03,Hull08}
have lately emerged as an effective framework to model business-relevant
entities, by combining in a holistic way their static and dynamic
aspects. Artifacts are characterized by an "information model", which maintains
the artifact data, and by a lifecycle that specifies the allowed ways to
progress the information model.  Among the different proposals for
artifact-centric process modelling, the Guard-Stage-Milestone (GSM) approach
has been recently proposed to model artifacts and their lifecycle in a
declarative, flexible way \cite{HDDF*11}. GSM is equipped with a formal
execution semantics \cite{DaHV13}, which unambiguously characterizes the
artifact progression in response to external events. Notably, several key
constructs of the emerging OMG standard on Case Management and Model Notation
\footnote{\url{http://www.omg.org/spec/CMMN/}} have been borrowed from GSM.

Despite the tight integration between the data and process component, the
artifact information model typically relies on relatively simple structures,
such as (nested) lists of key-value pairs.  This causes an abstraction gap
between the high-level, conceptual view that business stakeholders have of
domain-relevant entities and relations, and the low-level representation
adopted inside artifacts.  To overcome this problem, in \cite{CDLMS12} it is
proposed to enhance artifact systems with a Semantic Layer, constituted by a
full-fledged ontology linked to the artifact information models through mapping
specifications. On the one hand, the ontology provides a conceptual view of the
domain under study, and allows one to understand the evolution of the artifact
system at a higher level of abstraction. On the other hand, mapping
specifications allow one to connect the elements present in the Semantic Layer
with the concrete data maintained in the artifact information models, relying
on an approach recently proposed in the context of Ontology-Based Data Access
(OBDA) \cite{CDLL*09}.

To specify the ontology, we adopt the OWL~2~QL profile \cite{MCHW*12} of the
standard Web Ontology Language (OWL) \cite{BaEA12}, since it supports efficient
access to data while fully taking into account the constraints expressed in the
ontology.  Specifically, OWL~2~QL enjoys so-called \emph{first-order
 rewritability} of query answering \cite{CDLLR07}, which guarantees that
conjunctive queries posed over the ontology can be rewritten into first-order
queries that incorporate the ontological constraints, and thus do not require
further inference for query answering.  A rewritten query can then be
\emph{unfolded} with respect to the mappings, so as to obtain a query
formulated over the underlying data that can be directly evaluated so as to
obtain the so-called \emph{certain answers} to the original query over the
ontology \cite{PLCD*08}.

We follow here an approach that is similar to the one proposed in
\cite{CDLMS12}, and that is based on specifying in terms of the Semantic Layer
dynamic/temporal laws that the system should obey, and that need to be verified
according to the evolution in the underlying artifact layer.  However,
differently from \cite{CDLMS12}, in which the Semantic Layer is mainly used to
\emph{govern} the progression of artifacts, by forbidding the execution of
actions that would lead to violate the constraints in the ontology, here we are
primarily interested in exploiting the Semantic Layer to ease the specification
of the dynamic/temporal laws.
%
In this light, we extend the technique provided in \cite{CDLMS12}
% to specify rich temporal properties expressed over the Semantic Layer, and
% verify them according to the evolution in the underlying artifact layer.
% Specifically, the extension relies
by relying on a more expressive verification formalism, which supports
first-order epistemic queries embedded into an expressive temporal language,
the first-order $\mu$-calculus \cite{Emer96b}, while allowing for
quantification across states.  The latter makes it possible to predicate over
the temporal evolution of individuals, and thus represents an enhancement that
is fundamental for capturing many practical scenarios (cf.\
Section~\ref{sec:caseStudy}).

We then concretize this formal framework by relying on GSM as the artifact
model, and by exploiting state of the art technologies, on the one hand for
dealing with the ontology and the mappings, and on the other hand for
performing verification.  Specifically, we have developed the OBGSM tool (see
Section~\ref{sec:obgsmtool}), which is able to reformulate temporal properties
expressed over the ontology in terms of the underlying GSM information model,
and which adopts the state of the art OBDA system Quest \cite{RoCa12b} to
efficiently rewrite and unfold the epistemic queries embedded in the temporal
property to verify.  For the actual verification task, we rely on the recently
developed GSMC model checker for GSM \cite{BeLP12b}, which is the only model
checker currently available that is able to verify temporal formula over
artifact systems.  GSMC adopts as temporal formalism a variant of the
first-order branching time logic CTL \cite{ClGP99} with a restricted form of
quantification across states\footnote{Note that CTL can be expressed in the
 alternation-free fragment of the $\mu$-calculus \cite{Dam92,Emer96b}.}.  The
restrictions imposed by GSMC made it necessary to suitably accommodate the
mapping language and the temporal formalism over the Semantic Layer so as to
ensure that the temporal formulas resulting from rewriting and unfolding can be
effectively processed by GSMC.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> submitted/2-preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

OWL~2~QL is a profile\footnote{In W3C terminology, a \emph{profile} is a
 sublanguage defined by suitable syntactic restrictions.} of the Web Ontology
Language OWL~2 standardized by the W3C.
% In W3C terminology, a \emph{profile} is a sublanguage of the full OWL~2,
% defined by suitable syntactic restrictions.
OWL~2~QL is specifically designed for building an ontology layer to
wrap possibly very large data sources.
% Notably, it allows for query answering over ontologies with the same data
% complexity as plain SQL query evaluation over relational databases.
Technically, OWL~2~QL is based on the description logic \dlliter, which is a
member of the \dllite family \cite{CDLLR07}, designed specifically for
effective ontology-based data access, and which we adopt in the following.

In description logics (DLs) \cite{BCMNP03}, the domain of interest is modeled
by means of \emph{concepts}, representing classes of objects, and \emph{roles},
representing binary relations between objects\footnote{For simplicity of
 presentation, we do not distinguish here between roles, corresponding to OWL~2
 object properties, and attributes, corresponding to OWL~2 data properties (see
 \cite{CDLL*09}).  But all our results would carry over unchanged.}
%%
In \dlliter, concepts $C$ and roles $U$
% are formed according
obey to the following syntax:
\[
  B ~::=~  N ~\mid~ \SOMET{U}
  \qquad\qquad
  C ~::=~  B ~\mid~ \SOME{U}{B}
  \qquad\qquad
  U ~::=~  P ~\mid~ \INV{P}
  %% V &~::=~&  U ~\mid~ \NOT U
\]
$P$ denotes a \emph{role name}, and $\INV{P}$ an \emph{inverse role}, which
swaps the first and second components of $P$.  $N$ denotes a \emph{concept
 name}, and $B$ a \emph{basic concept}, which is either simply a concept name,
or the projection of a role $P$ on its first component ($\SOMET{P}$) or its
second component ($\SOMET{P^-}$).  In the concept $\SOME{U}{B}$, the projection
on the first (resp., second) component of $U$ can be further qualified by
requiring that the second (resp., first) component of $U$ is an instance of the
basic concept $B$.

In DLs, domain knowledge is divided into an intensional part, called
\emph{TBox}, and an extensional part, called \emph{ABox}.  Specifically, a
\dlliter \emph{ontology} is a pair $(\T,\A)$, where the TBox $\T$ is a finite
set of (concept and role) \emph{inclusion assertions} of the forms $B\ISA C$
and $U_1\ISA U_2$, and of \emph{disjointness assertions} of the form
$\disjoint{B_1}{B_2}$ and $\disjoint{U_1}{U_2}$.  Instead, the ABox $\A$ is a
finite set of \emph{facts} (also called membership assertions) of the forms
$N(c_1)$ and $P(c_1,c_2)$, where $N$ and $P$ occur in $\T$, and $c_1$ and $c_2$
are constants.
% We denote with $\const{\A}$ the set of constants appearing in $\A$.

The semantics of a \dlliter ontology is given in terms of first-order
\emph{interpretations} $\I=(\dom,\Int{\cdot})$, where $\dom$ is the
interpretation domain and $\Int{\cdot}$ is an interpretation function that
assigns to each concept $C$ a subset $\Int{C}\subseteq\dom$ and to each role
$U$ a binary relation $\Int{U}\subseteq\dom\times\dom$, capturing the intuitive
meaning of the various constructs (see~\cite{CDLLR07} for details).
%%
%% Notice that in \dlliter the unique name assumption is immaterial, since
%% there is no way of deducing facts about equality.
%%
An interpretation that satisfies all assertions in $\T$ and $\A$ is called a
\emph{model} of the ontology $(\T,\A)$, and the ontology is said to be
\emph{satisfiable} if it admits at least one model.
%%% Probably not needed
% We also say that $A$ is \emph{$T$-consistent} if $(T,A)$ is satisfiable, i.e.,
% admits at least one model, otherwise we say $A$ is \emph{$T$-inconsistent}.

\smallskip
\noindent
\textbf{Queries.}  As usual (cf.\ OWL~2~QL), answers to queries are formed by
terms denoting individuals explicitly mentioned in the ABox.  The \emph{domain
 of an ABox} $A$, denoted by $\adom{A}$, is the (finite) set of terms appearing
in $A$.
%%
A \emph{union of conjunctive queries} (UCQ) $q$ over a KB $(T,A)$ is a FOL
formula of the form
%%
%% $\exists\vec{y}_1\per\conj_1(\vec{x},\vec{y}_1) \lor\cdots\lor
%% \exists\vec{y}_n\per\conj_n(\vec{x},\vec{y}_n)$,
%%
$\bigvee_{1\leq i\leq n}\exists\vec{y_i}\per\conj_i(\vec{x},\vec{y_i})$ with free
variables $\vec{x}$ and existentially quantified variables
$\vec{y}_1,\ldots,\vec{y}_n$.  Each $\conj_i(\vec{x},\vec{y_i})$ in
$q$ is a conjunction of atoms of the form $N(z)$, $P(z,z')$, where $N$
and $P$ respectively denote a concept and a role name occurring in
$T$, and $z$, $z'$ are constants in $\adom{A}$ or variables in
$\vec{x}$ or $\vec{y_i}$, for some $i\in\{1,\ldots,n\}$.
%
%% Notice that since UCQs are defined over a TBox $T$, the special
%% role $\eq{}{}$ cannot appear here.
%%
The \emph{(certain) answers} to $q$ over $(T,A)$ is the set $\ans{q,T,A}$ of
substitutions %\footnote{As customary, we can view each substitution simply as a
 %tuple of constants, assuming some ordering of the free variables of $q$.}
$\sigma$ of the free variables of $q$ with constants in $\adom{A}$ such that
$q\sigma$ evaluates to true in every model of $(T,A)$.
%%
If $q$ has no free variables, then it is called \emph{boolean} and its certain
answers are either $\true$ or $\false$.

We compose UCQs using ECQs, i.e., queries of the query language
\textit{EQL-Lite}(UCQ)~\cite{CDLLR07b}, which is the FOL query language whose
atoms are UCQs evaluated according to the certain answer semantics above. An
\emph{ECQ} over $T$ and $A$ is a possibly open formula of the form
\[
  Q ~:=~
  [q] ~\mid~
%[\eq{x}{y}] ~\mid~
\lnot Q ~\mid~ Q_1\land Q_2 ~\mid~
  \exists x\per Q
\]
where $q$ is a UCQ.
%
% where $q$ denotes a UCQ over $\T$ and $\C$, with the proviso that
% every free variable of a negative subquery, i.e., of the form $\lnot
% Q$, must occur in a positive subquery (to guarantee
% range-restriction).
%%
%%%%%%%%%%%%%%%%%%%%%%%
% First of all, notice that what is asserted in $\eq$ is \emph{known}
% to be valid in any model of the ontology. Intuitively, $\eq(t_1,
% t_2)$ implies that $t_1$ and $t_2$ reference the same domain object.
%%%%%%%%%%%%%%%%%%%%%%%
The \emph{answer to $Q$ over $(\T,\A)$}, is the set $\Ans{Q,\T,\A}$ of
tuples of constants in $\adom{A}$ defined by composing the certain
answers $\ans{q,T,A}$ of UCQs $q$ through first-order constructs, and
interpreting existential variables as ranging over $\adom{A}$.
% $ \Ans{\exists x \per Q,T,A} =\bigcup_{t \in\adom{A}}\,
%      \Ans{Q_{x/t},T,A}$,
% % as follows:
% % \[
% %   \begin{array}{r@{~}c@{~}l}
% %     \Ans{[q],T,A} &=& \ans{q,T,A}\\
% %     \Ans{[\eq{x}{y}],T,A} &=& \{\tup{x,y} \in \adom{A} \mid (T,A)\models
% %     x\=y\}\\
% %     %% \ans{\eq(x,y),T,A};\\
% %     \Ans{\lnot Q,T,A} &=& \adom{A} \setminus \Ans[]{Q,T,A}\\
% %     \Ans{Q_1 \land Q_2,T,A} &=& \Ans{Q_1,T,A} \cap \Ans{Q_2,T,A}\\
% %   \Ans{\exists x \per Q,T,A} &=&\bigcup\limits_{t \in\adom{A}}\,
% %     \Ans{Q_{x/t},T,A}\\
% %  \end{array}
% % \]
%  where $Q_{x/t}$ is obtained from $Q$ by substituting each
%  occurrence of $x$ with $t$.

Finally, we recall that \dlliter enjoys the \emph{FO rewritability} property,
which states that for every UCQ $q$, $\ans{q,\T,\A} =
\ans{\textsc{rew}(q),\emptyset,\A}$, where $\textsc{rew}(q)$ is a UCQ computed by the
reformulation algorithm in \cite{CDLL*09}. Notice that this algorithm can be
extended to ECQs \cite{CDLLR07b}, and that its effect is to ``compile away''
the TBox. Similarly, ontology satisfiability is FO rewritable for \dlliter
TBoxes \cite{CDLL*09}, which states that for every TBox $\T$, there exists a
boolean first-order query $\qunsat{\T}$ such that for every non-empty ABox
$\A$, we have that $(\T,\A)$ is satisfiable iff
$\ans{\qunsat{\T},\T,\A}=\false$.


% \todo[inline]{\textbf{TODO:} Explain OBDA?}

\smallskip
\noindent
\textbf{Ontology-Based Data Access (OBDA).}
\label{sec:OBDASystem}
%%
In an OBDA system, a relational database is connected to an ontology
representing the domain of interest by a mapping, which relates database values
with values and (abstract) objects in the ontology (cf.\ \cite{CDLL*09}).
%
In particular, we make use of a countably infinite set  $\VALUE$ of
values and a set $\Lambda$ of function symbols, each with an
associated arity. We also define the set $\CONST$ of constants as the
union of  $\VALUE$ and the set
$\{f(d_1,\ldots,d_n) \mid f \in \Lambda \text{ and } d_1,\ldots,d_n \in
\VALUE \}$ of \emph{object terms}.

Formally, an OBDA system is a structure $\obdaSym = \obdaTup$, where:
\begin{inparaenum}[\it (i)]
\item $\DBschema =\set{R_1, \ldots, R_n}$ is a database schema, constituted by
  a finite set of relation schemas;
  % and $\DBinit$ is the initial database instance that conforms to
  % $\DBschema$.
\item $\TBox$ is a \dlliter TBox;
\item $\mapping$ is a set of mapping assertions, each of the form
%\begin{center}
  $\map{\Phi(\vec{x})}{\Psi(\vec{y},\vec{t})}$,
%\end{center}
  where:
  \begin{inparaenum}
  \item $\vec{x}$ is a non-empty set of variables,
  \item $\vec{y} \subseteq \vec{x}$,
  \item $\vec{t}$ is a set of object terms of the form $f(\vec{z})$, with $f
    \in \Lambda$ and $\vec{z} \subseteq \vec{x}$,
  \item $\Phi(\vec{x})$, which also called as \emph{source query}, is an arbitrary SQL query over $\DBschema$, with
    $\vec{x}$ as output variables, and
  \item $\Psi(\vec{y},\vec{t})$, which also called as \emph{target query}, is a CQ over $\TBox$ of arity $n >0$ without
    non-distinguished variables, whose atoms are over the variables $\vec{y}$
    and the object terms $\vec{t}$.
  \end{inparaenum}
\end{inparaenum}

Given a database instance $\DBinst$ made up of values in $\VALUE$ and
conforming to schema $\DBschema$, and given a mapping $\mapping$, the
\emph{virtual ABox} generated from $\DBinst$ by a mapping assertion
$m=\map{\Phi(x)}{\Psi(y,t)}$ in $\mapping$ is
$m(\DBinst)=\bigcup_{v\in\evaluate(\Phi,\DBinst)} \Psi[x/v]$, where
$\evaluate(\Phi,\DBinst)$ denotes the evaluation of the SQL query $\Phi$ over
$\DBinst$, and where we consider $\Psi[x/v]$ to be a set of atoms (as opposed
to a conjunction).  The ABox generated from $\DBinst$ by the mapping $\mapping$
is $\mapping(\DBinst)=\bigcup_{m \in \mapping} m(\DBinst)$.
%
Notice that $\adom{\mapping(\DBinst)} \subseteq \CONST$.
As for ABoxes, the active domain $\adom{\DBinst}$
of a database instance $\DBinst$ is the set of values occurring in
$\DBinst$. Notice that $\adom{\DBinst} \subseteq \VALUE$.
%
% Given a database instance $\DBinst$ (an ABox $\ABox$ resp.), its active
% domain $\adom{\DBinst}$ ($\adom{\ABox}$) is the subset of $\VALUE$ (of
% \todo{Dobbiamo fissare il dominio degli oggetti!}\ldots) such that
% $c\in\adom{\DBinst}$ iff $c$ occurs in $\DBinst$ ($c\in\adom{\ABox}$ iff $c$
% occurs in $\ABox$).
%
Given an OBDA system $\obdaSym = \obdaTup$ and a database instance
$\DBinst$ for $\DBschema$, a \emph{model} for $\obdaSym$ wrt $\DBinst$ is a
model of the ontology $(\TBox,\mapping(\DBinst))$. We  say that
$\obdaSym$ wrt $\DBinst$ is satisfiable if it admits a model wrt $\DBinst$.

A UCQ $q$ over an OBDA system $\obdaSym = \obdaTup$ and a relational
instance $\DBinst$ for $\DBschema$ is simply an UCQ over
$(\TBox,\mapping(\DBinst))$. To compute the certain answers of $q$
over $\obdaSym$ wrt $\DBinst$, we follow the standard three-step approach~\cite{CDLL*09}:
\begin{inparaenum}[\it (i)]
\item $q$ is \emph{rewritten} to compile away $\TBox$, obtaining $q_r =
  \rew{q,\TBox}$;
\item the mapping $\mapping$ is used to \emph{unfold} $q_r$ into a query over
  $\DBschema$, denoted by $\unfold{q_r}{\mapping}$, which turns out to be an
  SQL query \cite{PLCD*08};
\item such a query is executed over $\DBinst$, obtaining the certain answers.
\end{inparaenum}
For an ECQ, we can proceed in a similar way, applying the rewriting and
unfolding steps to the embedded UCQs.  It follows that computing certain
answers to UCQs/ECQs in an OBDA system is FO rewritable. Applying the
unfolding step to $\qunsat{\TBox}$, we obtain also that satisfiability in
$\obdaSym$ is FO rewritable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \todo[inline]{\textbf{TODO:} Explain GSM? }


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> submitted/3-sas.tex <==
\section{Semantically-enhanced Artifact Systems}
\label{sec:sas}

In this section we introduce Semantically-enhanced Artifact Systems ($\sgds$s),
which generalize the framework of Semantically-Governed Data-Aware Processes
(SGDAPs) presented in \cite{CDLMS12}.


Intuitively, \sgds models systems in which artifacts progress according to
their lifecycles, and in which the evolution of the entire system is understood
through the conceptual lens of an OWL~2~QL ontology. In accordance with the
literature \cite{DHPV09}, it is assumed that artifacts are equipped with a
relational information model. More specifically, a \sgds is constituted by:
\begin{inparaenum}[\it (i)]
%
\item A \emph{Relational Layer}, which account for the
  (relational) information models of the artifacts, and which employs a
  global transition relation to abstractly capture the step-by-step
  evolution of the system as a whole.
%
\item A \emph{Semantic Layer}, which contains an OWL~2~QL ontology
  that conceptually accounts for the domain under study.
%
\item A set of \emph{mapping assertions} describing how to
  virtually project data concretely maintained at the Relational Layer
  into concepts and relations modeled in the Semantic Layer, thus
  providing a link between the artifact information models and the ontology.
%
  % We assume that the Artifact Layer exploits relational databases to
  % maintain the data of interest, and can be hence queried by means
  % of SQL statements; in this context context, each mapping assertion
  % relates an arbitrary (SQL) query over the databases of the
  % artifacts to a set of atoms whose predicates are the concepts and
  % roles of the ontology, and whose arguments are terms built using
  % specific function symbols applied to the answer variables of the
  % SQL query.  Such mappings specify how to populate the elements of
  % the ontology
  % from the data in the relational database, and the function symbols
  % are used to construct (abstract) objects (which we call
  % \emph{object
  % terms}) from the concrete values retrieved from the database.
%
\end{inparaenum}
%
% Since the main focus of this investigation is on how data are
% manipulated at the Artifact Layer and understood/governed at the
% Semantic Layer, we assume, as done for $\dcds$s and $\kbds$s, that
% the artifact databases are combined into a unique database
% maintaining the whole information present at the Artifact Layer,
% which is then referred to as the \emph{Relational Layer}.
%
%


\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{imgs/rts-sts2}
\vspace*{-6mm}
\caption{\sgds illustration \label{fig:evolution}}
\end{figure}


%\todo[inline]{\textbf{TODO:} Explain SAS's components formal definition}

In the following, we assume a countably infinite set of values $\VALUE$.
Formally, a \sgds $\sgdsSym$ is a tuple
$\sys = \tup{\DBschema,\DBinit,\F, \TBox, \mapping}$, where:
%
\begin{inparaenum}[\it (i)]
%
\item $\DBschema$ is a database schema that incorporates the schemas
  of all artifact information models present in the Relational Layer;
%
\item $\DBinit$ is a database instance made up of
  values in $\VALUE$ and conforming to $\DBschema$, which represents
  the initial state of the Relational Layer,;
%
\item $\F\subseteq \Instances\times \Instances$ is the transition
  relation that describes the overall progression mechanism of the
  Relational Layer, where $\Instances$ is the set of all instances
  made up of values in $\VALUE$ and conforming to $\DBschema$;
%
% \item $\kabkb = \tup{\TBox,\mapping}$ is the knowledge component of
%   $\KA$, constituted by a \dllitea;
%
\item $\TBox$ is a $\dlliter$ TBox; 
%
\item $\mapping$ is a set of mapping assertions that connect $\DBschema$
  to $\TBox$, following the approach described in
  Section~\ref{sec:preliminaries}.
%
\end{inparaenum}
%
By observing that the triple $\tup{\DBschema,\TBox,\mapping}$
constitutes, in fact, an OBDA system, we notice that $\sys$ can be
considered as an OBDA system equipped with a transition relation that
accounts for the dynamics of the system at the level of $\DBschema$,
starting from the initial state $\DBinit$.

% Roughly speaking, the components $\DBschema,\DBinit,\F$ together
% constitute the relational layer and the components $\TBox, \mapping$
% together build up the Semantic Layer.
% %
% Also notice that, in fact the components $\DBschema,\TBox,\mapping$
% constitute OBDA system.
% For an overall picture providing the intuition for $\sgds$s, see
% Figure~\ref{fig:verification}.


%


\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/3.1-executionSemantic.tex <==
\subsection{Execution Semantics}
\label{sec:executionSemantic}
% \todo[inline]{\textbf{TODO:} 
%   - Explain SAS's process/action execution semantic? \\
% }
% \todo[inline]{\textbf{TODO:} \\
% - Explain SAS's semantics in terms of transition systems (Semantic
% and artifact layer TS?)  }






The execution semantics of a $\sgds$ \sys is provided by means of transition
systems. While the temporal structure of such transition systems is
fully determined by the transition relation of \sys, the content of
each state in the transition system depends on whether the dynamics of
$\sgds$s are understood directly at the Relational Layer, or through
the conceptual lens of the Semantic Layer ontology. In the former
case, each state is associated to a database instance that represents
the current snapshot of the artifact information models, whereas in
the latter case each state is associated to an ABox that represents
the current state of the system, as understood by the Semantic Layer. 

Following this approach,  the execution semantics of $\sgdsSym$ is captured in terms of two
transition systems, one describing the allowed evolutions at the
Relational Layer (\emph{Relational Transition System - RTS}),
and one abstracting them at the Semantic Layer (\emph{Semantic
  Transition System} - STS). Figure~\ref{fig:evolution} provides a
graphical intuition about the RTS and STS, and their
interrelations. 

%%
% The first transition system has the form of an RTS
% (cf.~Section~\ref{sec:rel-ts}), whereas the second has the form of
% an STS (cf.~Section~\ref{sec:sem-ts}).
%%
% \noindent
% \textbf{RTS.}  The RTS $\TSAsym_\sgdsSym$ of the \sgds $\sgdsSym=\tup{\DBschema,\DBinit,\F, \TBox, \mapping}$ is
% defined as $\TSAtup$, where $\TSAs$, $\TSAt$ and $\db$ are defined by
% simultaneous induction as the smallest sets such that $s_0 \in \TSAs$,
% with $\db(s_0) = \DBinit$, and satisfying the following
% property. Given $s \in \TSAs$, consider every database instance
% $\DBinst'$ such that $\tup{\db(s),\DBinst'} \in \F$. Then:
% \begin{compactitem}
% \item[\it (i)] if there exists $s' \in \TSAs$ such that $\db(s') =
%   \DBinst'$, then $s \TSAt s'$;
%   \item[\it (ii)] otherwise, if $\obdaSym =
%     \tup{\DBschema,\TBox,\mapping}$ is \emph{satisfiable} wrt
%     $\DBinst'$, then $s' \in \TSAs$, $s \TSAt s'$ and $\db(s') =
%     \DBinst'$, where $s'$ is a fresh state.
% \end{compactitem}
% We observe that the satisfiability check done in the last step of the
% RTS construction accounts for \emph{semantic governance}.
%%

\smallskip
\noindent
\textbf{RTS.} 
Given a \sgds $\sgdsSym=\tup{\DBschema,\DBinit,\F, \TBox, \mapping}$,
its RTS $\TSAsym_\sgdsSym$ is defined as a tuple $\TSAtup$, where:
\begin{inparaenum}[\it (i)]
\item  $\TSAs$ is a set of states,
\item $s_0 \in \TSAs$,
\item $\db$ is a function that, given a state in $\TSAs$, returns a
  corresponding database instance (conforming to $\DBschema$),
\item $\TSAt \subseteq \TSAs \times \TSAs$ is the transition relation.
\end{inparaenum} 
The components $\TSAs$, $\TSAt$ and $\db$ of $\TSAsym_\sgdsSym$ are
defined by
simultaneous induction as the smallest sets satisfying the following conditions:
\begin{compactitem}
\item $\db(s_0)  = \DBinit$;
\item for every databases instance $\DBinst'$ such that
  $\tup{\db(s),\DBinst'} \in \F$:
   \begin{compactitem}
   \item if there exists $s' \in \TSAs$ such that $\db(s') =
     \DBinst'$, then $s \TSAt s'$;
   \item otherwise, if $\obdaSym = \tup{\DBschema,\TBox,\mapping}$ is
     \emph{satisfiable} wrt $\DBinst'$, then $s' \in \TSAs$, $s \TSAt
     s'$ and $\db(s') = \DBinst'$, where $s'$ is a fresh state.
   \end{compactitem}
\end{compactitem}

%  such that $s_0 \in \TSAs$,
% with $\db(s_0) = \DBinit$, and satisfying the following
% property. Given $s \in \TSAs$, consider every database instance
% $\DBinst'$ such that $\tup{\db(s),\DBinst'} \in \F$. Then:
% \begin{compactitem}
% \item[\it (i)] if there exists $s' \in \TSAs$ such that $\db(s') =
%   \DBinst'$, then $s \TSAt s'$;
% \item[\it (ii)] otherwise, if $\obdaSym =
%   \tup{\DBschema,\TBox,\mapping}$ is \emph{satisfiable} wrt
%   $\DBinst'$, then $s' \in \TSAs$, $s \TSAt s'$ and $\db(s') =
%   \DBinst'$, where $s'$ is a fresh state.
% \end{compactitem}
%%

\noindent
The satisfiability check done in the last step of the
RTS construction accounts for the semantic \emph{governance}
(cf.~Section \ref{sec:introduction}): a transition is preserved in the
RTS only if the target state does not violate any ontological
constraints of the Semantic Layer, otherwise it is rejected \cite{CDLMS12}.

\smallskip
\noindent
\textbf{STS.}  
Given a \sgds $\sgdsSym=\tup{\DBschema,\DBinit,\F, \TBox, \mapping}$,
its STS $\TSSsym_\sgdsSym$ is defined as a tuple $\TSAtup$, which is
similar to an RTS, except from the fact that states are attached to
ABoxes, not database instances.
 In particular, $\TSSsym_\sgdsSym$ is defined as a
``virtualization'' of the RTS $\TSAsym_\sgdsSym=\TSAtup$ at the
Semantic Layer: it maintains the structure of $\TSAsym_\sgdsSym$
unaltered, reflecting that the progression of the system is determined
at the Relational Layer, but it associates each state to a virtual
ABox obtained from the application of the mapping specification
$\mapping$ to the database instance associated by $\TSAsym_\sgdsSym$
to the same state.  Formally, the transition relation $\mapping$ is
equivalent to the one of the $\sgdsSym$, and the $\abox$ function of
$\TSSsym_\sgdsSym$ is defined as follows: for each $s \in \TSSs$, 
$\abox(s) = \mapping(\db(s))$.

% \noindent
% \textbf{STS.}  The STS $\TSSsym_\sgdsSym$ of $\sgdsSym$ is defined as
% $\TSStup$, where $\TBox$ is the TBox of $\sgdsSym$. In particular,
% $\TSSsym_\sgdsSym$ is defined as a ``virtualization'' of the RTS
% $\TSAsym_\sgdsSym=\TSAtup$ at the Semantic Layer: it maintains the
% structure of $\TSAsym_\sgdsSym$ unaltered, reflecting that the
% progression of the system is determined at the Relational Layer, but
% it associates each state to a virtual ABox obtained from the
% application of the mapping specification $\mapping$ to the database
% instance associated by $\TSAsym_\sgdsSym$ to the same state.
% Formally, the $\abox$ function of $\TSSsym_\sgdsSym$ is defined as
% follows: for each $s \in \TSSs$ with $\db(s) = \DBinst$, $\abox(s) =
% \mapping(\DBinst)$.
%%


%%
% Figure~\ref{fig:rts-sts} provides a pictorial intuition of the two
% transition systems and their interconnection.

%\begin{figure}[!t]
%\centering
%\includegraphics[width=.7\textwidth]{imgs/rts-sts}
%\caption{Relationship between the RTS and STS of an \sgds $\sgdsSym$}
%\label{fig:rts-sts}
%\end{figure}

%The STS $\TSSsym_\sgdsSym$ allows us to define the \emph{verification}
%problem for a \sgds, i.e., verifying whether a
%%\emph{$\mulpdl$/$\muladl$ 
%\emph{$\muladl$ closed formula $\Phi$ holds for the $\sgds$
% $\sgdsSym$}: $\TSSsym_\sgdsSym \models \Phi$.  

% This, in turn, allows us to tackle the \emph{conformance} problem of
% $\TSSsym_\sgdsSym$ wrt the dynamic laws $\kabaction$ of a KAB $\KA =
% \tup{\kabkb,\kabaction}$: $\TSSsym_\sgdsSym$ conforms to
% $\kabaction$ if
%\[\TSSsym_\sgdsSym \models \bigwedge_{\Phi_i \in \kabaction} \Phi_i\]

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/4-verification.tex <==
\section{Verification of Semantically-Enhanced Artifact Systems}
\label{sec:verification}
Given a \sgds \sgdsSym, we are interested in studying verification of semantic
dynamic/temporal properties specified over the Semantic Layer, i.e., to be
checked against the STS $\TSSsym_\sgdsSym$. As verification formalism, we
consider a variant of first-order $\mu$-calculus \cite{Emer96b,Stir01},
called $\muladl$ \cite{BCMD*13,CKMSZ13}. We observe that $\mu$-calculus is one
of the most powerful temporal logics: it subsumes LTL, PSL, and CTL*
\cite{ClGP99}. The logic $\muladl$ extends propositional $\mu$-calculus by
allowing to query the states of the STS using the first-order epistemic queries
introduced in Section~\ref{sec:preliminaries}. In $\muladl$, first-order
quantification is restricted to objects that are present in the current ABox,
and can be used to relate objects across states.
%
The syntax of \muladl is as follows:
%{\footnotesize
\[
  \Phi ::= Q ~\mid~ \lnot \Phi ~\mid~ \Phi_1 \land \Phi_2 ~\mid~ \exists
  x.\inadom(x) \land \Phi ~\mid~ \DIAM{\Phi} ~\mid~ Z ~\mid~ \mu Z.\Phi
\]
%}%
%%
Where $Q$ is an ECQ over $\TBox$, $Z$ is a second-order variable denoting a
0-ary predicate, $\mu$ is the least fixpoint operator, and the special
predicate $\inadom(x)$ is used to indicate that $x$ belongs to the current
active domain, i.e., it is mentioned in some concept or role of the current
ABox. For a detailed semantics of \muladl, refer to
\cite{BCMD*13,CKMSZ13}.

% \todo{Two examples of properties?}
 
\begin{comment}
%%
We make use of the usual abbreviation, including $\forall x.\inadom(x) \limp
\Phi = \neg (\exists x.\inadom(x) \land \neg \Phi)$.

To define the semantics of $\muladl$ we resort to STSs.
Let $\Upsilon = \TSStup$ be an STS.
% $\mf{A}=\Upsilon_\S$ be the transition system for $\S=(\T,\A_0,\R,
% \Pi)$. We denote by $\Sigma_\mf{A}$ the states of $\mf{A}$.
Let $\vso$ be a predicate and individual variable valuation on $\Upsilon$,
i.e., a mapping from the predicate variables $Z$ to subsets of the
states $\TSSs$, and from individual variables to constants
in $\adom{\mapping(\DBinit)}$.
%
Then, we assign meaning to $\muladl$ formulas by associating to
$\Upsilon$ and $\vso$ an \emph{extension function} $\MODA{\cdot}$, which
maps $\muladl$ formulas to subsets of $\TSSs$.
%
The extension function  $\MODA{\cdot}$ is defined inductively as:

%\begin{figure}[t]
{\footnotesize{\[
  \begin{array}{rcl}
    \MODA{Q} &=& \{s \in \Sigma\mid \ans{Q\vfo,\db(s)} \}\\
    \MODA{\lnot \Phi} &=& \Sigma \setminus \MODA{\Phi} \\
    \MODA{\Phi_1 \land \Phi_2} &=&\MODA{\Phi_1}\cap\MODA{\Phi_2}\\
    \MODA{\exists x. \Phi} &=& \{ s \in \Sigma \mid\exists t. t \in
    \Delta\mbox{ and } s \in\MODAX{\Phi}{[x/t]}\}\\
    \MODA{\DIAM{\Phi}} &=& \{s \in \Sigma\mid\exists s'.s \Rightarrow s' \text{
     and } s' \in \MODA{\Phi}\} \\
    \MODA{Z} &=& \vso(Z)\\
    \MODA{\mu Z.\Phi} &=&
     \bigcap\{\S\subseteq\Sigma \mid \MODAZ{\Phi}{[Z/\S]} \subseteq \S
     \} \\
    % \MODA{\nu Z.\Phi} &=& \bigcup\{\S\subseteq\Sigma
    % \mid \S \subseteq \MODAZ{\Phi}{[Z/\S]}\}
     \MODA{\inadom(x)} &=&  \{s \in \Sigma\mid x/d \in \vfo \text{ implies }
     d \in \adom{\db(s)}\}
   \end{array}
\]
}}
%  \caption{\label{fig:mul-semantics} Semantics of $\mu\L$}
%\end{figure}

\end{comment}


Given a  \sgds \sgdsSym, we show that verification
of $\muladl$ properties over the STS $\TSSsym_\sgdsSym$ can be reduced
to verification of $\muladom$ \cite{CaDM13} properties over the RTS
$\TSAsym_\sgdsSym$, where $\muladom$ is a logic similar to $\muladl$,
except for the local formula $Q$, which is an (open) first-order query over the database
schema in the Relational Layer.

\begin{theorem}
\label{thm:verification}
For every \sgds \sgdsSym and \muladl property $\Phi$, there exists a
\muladom property $\Phi'$ such that $\TSAsym_\sgdsSym$ satisfies
$\Phi$ if and only if $\TSSsym_\sgdsSym$ satisfied $\Phi'$.
\end{theorem}

\begin{proof}[sketch]
The proof extends the one in \cite{CDLMS12}. We recap such a proof
here, and show how to extend it to the logic $\muladl$. 
The construction of $\Phi'$ is done by \emph{rewriting} and
\emph{unfolding} the $\Phi$, by suitably extending the
notions of rewriting and unfolding in OBDA to the case of temporal
properties \cite{PLCD*08}.

As for the rewriting step, the TBox $\TBox$ does not focus on the dynamics of the
system, but only on the information maintained by
$\sgdsSym$. Therefore, the rewriting of $\Phi$ wrt
the TBox $\TBox$ is done by separating the treatment of the
dynamic part, which is simply maintained unaltered, to the one of the
embedded ECQs, which is handled as in standard OBDA.

The unfolding step is managed in a similar way. Both $\TSSsym_\sgdsSym$ and $\TSAsym_\sgdsSym$
have the same structure, reflecting that the dynamics
of the SAS are determined at the Relational
Layer. Hence, the unfolding of $\rew{\Phi,\TBox}$ is handled by
maintaining the dynamic component unaltered, and unfolding all the embedded ECQs wrt the
mapping assertion $\mapping$. The correctness of this approach has
been proven in \cite{CDLMS12}, which however requires here to extend
the proof to the following two cases, related to first-order quantification:
\begin{inparaenum}[\it (i)]
\item the unfolding of $\inadom(x)$;
\item the unfolding of quantification across states, i.e., $\exists
  x.\inadom(x) \land \Phi$.
\end{inparaenum}
As for $\inadom(x)$, it can
be defined in terms of the following UCQ, which can then be unfolded
in the usual way:
{\footnotesize{
\[
\inadom(x) \equiv \bigvee_{N \text{ in } \TBox} N(x) \lor \bigvee_{P \text{ in } \TBox}
(P(x,\_) \lor P(\_,x))
\]
}}%
%
Quantification across states is dealt as in standard OBDA, i.e.:
{\small{
\begin{align*}
  \unfold{\exists x.\inadom(x) \land \Phi}{\mapping} =
  \textstyle\bigvee_{(f/n) \in \skolem(\mapping)} &\exists
  x_1,\ldots,x_n. 
  \unfold{\inadom(f(x_1,\ldots,x_n))}{\mapping} \\
  &\land \unfold{\Phi[x/f(x_1,\ldots,x_n)]}{\mapping}
\end{align*}
}}%
where $\skolem(\mapping)$ is the set of function symbols used to
construct object terms in $\mapping$. To conclude the proof, we need
to observe that the unfolded formula is in $\muladom$, i.e., it
preserves the property that quantification ranges over the current
active domain. This can be easily confirmed by noticing that a live
object term in a state of $\TSSsym_\sgdsSym$ can only be produced starting from
live values in the corresponding state of
$\TSAsym_\sgdsSym$. 
% that is live in a given state of the STS can be only produced starting from live values in the corresponding state of the RTS. Consequently, even if live(x1), ...live(xn) are not syntactically produced by the unfolding of live(f(x1,...,xn)), they are implied by the obtained formula.

% This approach shows that the verification problem for $\sgds$s can be
% reduced to a verification problem directly posed over the Relational
% Layer only. 

\end{proof}

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/5-sasInstantiation.tex <==
\section{SAS Instantiation: The OBGSM Tool}
\label{sec:obgsmtool}

\input{5.1-GSM}

\smallskip
\noindent
\textbf{The Ontology-Based GSM (OBGSM) Tool. } \xspace
\begin{comment}
\todo[inline]{\textbf{TODO:} \\
- Briefly introduce GSM (or put it in the preliminary?) \\
- Briefly Explain about GSMC and the formula it accepts?\\
- Explain about the temporal property we consider in OBGSM ($CTL_?$)
\\
- Describe the OBGSM architecture ( The components and their
interactions ). I'm not sure if we have enough space to describe the
input temporal property and input mapping syntax. In fact, we might
not need it, put it on some kind of technical report?
}
\end{comment}
%
%
% In Section~\ref{sec:sas}, we have introduced $\sgds$s as a formal
% framework for representing artifact systems with a Semantic
% Layer. In particular, we have focused our attention to the usage of
% lightweight Description Logics, belonging to the DL-Lite family, to
% conceptually capture the relevant domain entities and relationships
% at the Semantic Layer. Furthermore, in
% Section~\ref{sec:verification}, we have shown that, thanks to the FO
% rewritability of DL-Lite, verification of temporal properties and
% dynamic laws over the evolution of an artifact system understood
% through the lens of the Semantic Layer can be faithfully reduced to
% verification of properties directly carried out at the Artifact
% Layer.
%
%We continue the investigation of artifact systems equipped with a
%Semantic Layer, and show how the developed techniques can be exploited
%to effectively attack the verification problem, leveraging on:
\systemName exploits two already existing tools to provide its functionalities:
\begin{inparaenum}[\it (i)]
%
\item \ontop\footnote{\url{http://ontop.inf.unibz.it/}}, a JAVA-based
  framework for OBDA.
  % , and in particular the Quest reasoner, which is the component
  % dedicated to handle query rewriting and unfolding;
%
\item the \emph{GSMC model checker}, developed within the EU FP7 Project
  ACSI\footnote{``Artifact-Centric Service Interoperation'', see
   \url{http://www.acsi-project.eu/}} to verify GSM-based artifact-centric
  systems against temporal/dynamic properties \cite{BeLP12b}.
  % \todo{should we cite their ICSOC paper instead of ACSI deliverable
  % and should we say it's developed within ACSI?}.
%
\end{inparaenum}
An important observation is related to semantic governance in this
setting: since the construction of the RTS for GSM is handled
internally by GSMC, it is not possible (at least for the time being)
to prune it so as to remove inconsistent states. Therefore, in the
following we assume that all the states in the RTS are consistent with
the constraints of the Semantic Layer. This can be trivially achieved
by, e.g., avoiding to use negative inclusion assertions in the TBox,
which are the only source of inconsistency for OWL~2~QL. A more
elaborated discussion on this topic is included in Section~\ref{sec:discussion}.

The main purpose of \systemName is: given a temporal property specified over
the Semantic Layer of the system, together with mapping assertions whose
language is suitably shaped to work with GSMC, automatically rewrite and
unfold the property by producing a corresponding translation that can be directly
processed by the GSMC model checker.  This cannot be done by solely relying on
the functionalities provided by \ontop, for two reasons:
\begin{inparaenum}[\it (i)]
%
\item \systemName deals with temporal properties specified in a fragment of
  $\muladl$, and not just (local) ECQs;
%
\item the mapping assertions are shaped so as to reflect the specific query
  language supported by GSMC, guaranteeing that the rewriting and unfolding
  process produces a temporal property expressed in the input language of GSMC.
%
\end{inparaenum}
In particular, we note that GSMC is not able to process the entire
$\muladom$ logic, but only its CTL fragment, denoted by \ctla. This
requires also to restrict the $\muladl$ verification formalism
accordingly, in particular focusing on its CTL fragment, denoted by \ctladl.



As depicted in the Figure~\ref{fig:SystemArchitecture},
% \todo{I'll try to make more compact picture for this},
the workflow of \systemName is as follows:
%
\begin{inparaenum}[\it (i)]
%
\item The tool reads and parses the input
conceptual temporal property $\Phi$, the input ontology, and the input
mapping declaration $\mathcal{M}$.
%
\item It then \emph{rewrites} the input conceptual temporal property
  $\Phi$ based on the input ontology (TBox) in order to compile away
  the TBox.
%
% , in order to compile away the TBox.
%
  This step produces a \emph{rewritten temporal property}
  $\textsc{rew}(\Phi,\TBox)$.
%
\item The rewritten property  $\textsc{rew}(\Phi,\TBox)$ is \emph{unfolded} by
  exploiting $\M$.  The final temporal property $\Phi_{GSM} =
  \textsc{unfold}(\textsc{rew}(\Phi,\TBox), \mathcal{M})$
  obeys to the syntax expected by GSMC, and is such that verifying $\Phi$
  over the transition system of the GSM model under study
  after projecting its states into the Semantic Layer through $\M$,
  is equivalent to verifying $\Phi_{GSM}$ directly over the GSM model
  (without considering the Semantic Layer).
%
\item GSMC is invoked by passing $\Phi_{GSM}$ and the
  specification file of the GSM model under study.
%
\end{inparaenum}

Notice that the correctness of the translation is guaranteed by the fact that \systemName manipulates the local components of the query $\Phi$
according to the standard rewriting and unfolding algorithms, while
maintaining untouched the temporal structure of the property. This has
been proven to be the correct way of manipulating the property
(cf.~Theorem~\ref{thm:verification}). Furthermore, since the temporal
component of the formula is left untouched, it is guaranteed that
$\ctladl$ properties are rewritten and unfolded into corresponding
$\ctla$ properties.
%(cf.~Section~\ref{sec:rew-unfold-laws}).
% %The proof has been done for $\mulpdl$ and $\muladl$, and
% Since first-order $CTL$ with active domain quantification is a
% fragment of $\muladl$, the result directly applies also in our
% setting. This result also shows that \systemName can largely rely on
% state-of-the-art existing rewriting and unfolding techniques to
% manipulate the temporal properties.
%
% Indeed, \systemName exploits \ontop to accomplish this task, adding
% a last step to deal with the constructs that have been introduced
% for the mapping assertions, but that are not directly supported by
% GSMC. In particular, ``get'' statements are turned into
% corresponding existential quantifications, whereas variable
% assignments are managed by directly applying the constraints
% involving these variables to the attributes of the artifact
% information models, finally removing such additional variables.



%The implementation of \systemName is done in java. For some
%functionalities, it uses some components from \marianoSystem
%\footnote{\url{http://ontop.inf.unibz.it}} (An Ontology Based Data Access
%(OBDA) system which has \Quest \cite{OWLED-2012-obda} as it reasoner).
% The system architecture of \systemName is depicted in the
% Figure~\ref{fig:SystemArchitecture}.

\begin{figure}[tbp]
  \centering
  \hspace*{-3mm}\includegraphics[width=1.05\textwidth]{SystemArchitecture7}
  % \vspace*{-6mm}
  \caption{\systemName System Architecture \label{fig:SystemArchitecture}}
\end{figure}


%\smallskip
%\noindent
%\textbf{Specification of Conceptual Temporal Properties. }\xspace 

The verification language of \systemName relies on CTL, in accordance to the
input verification language of GSMC \cite{BeLP12b,ACSI-D2.2.3} with some
adjustment. Since we are querying over an OWL ontology, we rely for the local
query language on SPARQL, in accordance to the query language supported by
\ontop. More specifically, the syntax is as follows:

\vspace{-3mm}
{\footnotesize{
\begin{equation*}
\begin{split}
  \formula ~::=&~ [~\query~]
~\mid~ ( \formula )
~\mid~ \andTemp{\formula_1}{\formula_2}
~\mid~ \orTemp{\formula_1}{\formula_2}
~\mid~ \implTemp{\formula_1}{\formula_2}
~\mid~ \notTemp~\formula
~\mid~ \AG~\formula
~\mid~ \EG~\formula \\
~\mid&~ \AF~\formula
~\mid~ \EF~\formula
~\mid~ \AX~\formula
~\mid~ \EX~\formula
~\mid~ \Auntil{\formula_1}{\formula_2}
~\mid~ \Euntil{\formula_1}{\formula_2}  \\
%~\mid&~ \forallTemp \variables . \formula \\
% ~\mid&~ \existsTemp \variables . \formula
~\mid&~ \forallTemp\ \variables\ .\ \forallQuantification
~\mid~ \existsTemp\ \variables\ .\ \existsQuantification \\
%
\end{split}
\end{equation*}
%
\begin{equation*}
\begin{split}
%
\forallQuantification ~::=&~ \implTemp{[~\query~]}{\formula}
~\mid~ \forallTemp\ \variables\ .\ \forallQuantification
~\mid~ [~\query~] \\
%
%
\existsQuantification ~::=&~ \andTemp{[~\query~]}{\formula}
~\mid~ \existsTemp\ \variables\ .\ \existsQuantification
~\mid~ [~\query~] \\
%
%
\end{split}
\end{equation*}
}}%
where ``$\notTemp$'' denotes the negation, and $[\query]$ is
a %and $[\guard]$ are
\sparql \footnote{\url{http://www.w3.org/TR/sparql11-query/}} \sparqlSELECT
query, which only allows for:
\begin{inparaenum}[\it (i)]
\item prefixes declarations,
\item variables selections, and
\item a \sparqlWHERE clause that only contains triple patterns and some filters
  on variable/constant comparison.
\end{inparaenum}

The semantics of the temporal operators is the one of CTL \cite{ClGP99}.
% \cite{BaKG08}.
Additionally, we also impose the following restrictions on first-order
quantification:
%
\begin{inparaenum}[\it (i)]
%
\item Only closed temporal formulae are supported for verification.
%
\item Each first-order quantifier must be ``guarded'' in such a way that it
  ranges over individuals present in the current active domain.  This active
  domain quantification is in line with GSMC, and also with the \muladl
  logic. As attested by the grammar above, this is syntactically guaranteed by
  requiring quantified variables to appear in $[\query]$ according to the
  following guidelines:
  \begin{inparaenum}[\it (a)]
  \item $\forall \vec{x}. \query(\vec{x}) \limp \phi$
  \item $\exists \vec{x}. \query(\vec{x}) \land \phi$.
  \end{inparaenum}
%
% \[
%\begin{array}{l}
%\forall \vec{x}. \query(\vec{x}) \limp \phi\\
%\exists \vec{x}. \query(\vec{x}) \land \phi\\
%\end{array}
%\]
%
\item Quantified variables must obey to specific restrictions as
  follows: for each variable $y$ ranging over values, there must be at
  least one variable $x$ that ranges over object terms and that
  appears in the first component of the corresponding attribute (i.e.,
  $Attr(x,y)$ is present in the query, with $Attr$ being an attribute
  of the ontology), such that $x$ is quantified ``before'' $y$. For
  example, $\forall x. C(x) \implies \exists y. Attr(x.y)$ satisfies
  this condition, whereas $\exists y \exists x. Attr(x,y)$ does not.
%
\end{inparaenum}
%
%the quantification is restricted only into the current active domain.
%
%the quantification is restricted only to the quantification over
% \emph{objects terms} \todo{refer to object terms explanation in
% D2.3?} in the current \emph{active domain} \footnote{The set of
% individuals appear in the current (virtual) ABox in the
% ontology}. Consequently, quantification over value is not allowed.
%
%
These restrictions have been introduced so as to guarantee that the
conceptual temporal property can be translated into a corresponding
GSMC temporal property. In fact, GSMC poses several restrictions on
the way values (i.e., attributes of artifacts) can be accessed.

%\smallskip
%\noindent
%\textbf{Specification of the Input Mapping. } \xspace

The structure of the \systemName mapping language is mainly borrowed from
\ontop{}.
%
\begin{comment}
  The input mapping is started by the prefixes declaration. It defines
  URI (Uniform Resource Identifier) prefixes that will be used in the
  remainder of the file. An example of a prefix declaration is ``{\tt
    \footnotesize xsd: http://www.w3.org/2001/XMLSchema\#}'' which
  define the prefix ``{\tt \footnotesize xsd:}''.

  Within the mapping, we require that object terms only constructed by
  unary function symbols. As in \marianoSystem, function symbol in the
  mapping is represented by \emph{URI templates} (i.e., a preset
  format for URIs).  For example, the object term $f(x)$ is
  represented as {\tt\footnotesize
    <http://www.obgsm.inf.unibz.it/example/\#f\{x\}>}.
\end{comment}
%
%
% As the usage of function symbol in describing the object terms,
% during the processes, the variable {\tt x} in the URI template might
% be instantiated with a value and then it becomes a URI.
%
Each mapping assertion is described by three components:
\begin{inparaenum}[\it (i)]
\item {\tt \footnotesize mappingId}, which provides a unique identifier for the
  mapping assertion.
%
\item {\tt \footnotesize target}, which contains the \emph{target
    query} (query over ontology) with the syntax adopted from
  \marianoSystem.
\begin{comment}
 Technically, it is a CQ
  over the vocabulary of the ontology. We adopt the \marianoSystem\
  syntax in order to specify target query, which is in turn based on
  the Turtle\footnote{\url{http://www.w3.org/TR/turtle/}} syntax to
  represent RDF triples. Each atom in the CQ
  % \todo{check if it's ok to say CQ here, because there might be the
  % case that split will not
  % work anymore. Even if yes, should it be plain CQ (to avoid
  % equality)?}
  is in fact represented as an RDF-like triple template. 
  % \todo{need to refer to more detail explanation on mapping
  % structure, it's impossible to explain all here}
\end{comment}
%
\begin{comment}
Due to space limitation, we only
  provide intuition of the target query instead of explaining the
  whole detail. For example:
\begin{inparaenum}[\it (i)]
\item an atom $C(c(x))$, which is formed by a
  concept $C$ in the ontology and it has object term constructed by
  $c/1$, is represented as ``{\tt \footnotesize <"\&:;c\{\$x\}">
    rdf:type :C}'', where {\tt \footnotesize rdf:} is the prefix {\tt
    \footnotesize rdf: http://www.w3.org/1999/02/22-rdf-syntax-ns\#}
  and ``{\tt \footnotesize :}'' is a predefined prefix.
%
  % \todo{check if it's ok to say RDF-like triple}
  % There are three kinds of possible atoms in the target query:
%
\item an atom $R(r1(x), r2(y))$, which is formed by a role
  $R$ in the ontology and it has object term constructed by $r1/1$ and
  $r2/1$, is represented as ``{\tt \footnotesize <"\&:;r1\{\$x\}"> :R
    <"\&:;r2\{\$y\}">} ''.
%
\item an atom $A(att(x), integer(y))$, which is formed by an attribute
  $A$ in the ontology and it has object term constructed by $att/1$
  and $integer/1$, is represented as ``{\tt \footnotesize
    <"\&:;att\{\$x\}"> :A \$y\^{}\^{}xsd:integer .} '', where the
  second component of an attribute is a typed value. We use dedicated
  function symbols to wrap the value into an object term, ensuring
  that this choice does not overlap with any function symbol chosen
  for ``real'' object terms. In the example above, we use ``{\tt
    \footnotesize http://www.w3.org/2001/XMLSchema\#integer}'', but in
  general, we support the data types as in \marianoSystem.
%
\end{inparaenum}
\end{comment}
%
%###########################################################################################
%###########################################################################################
\item {\tt \footnotesize source}, which describes the \emph{source
    query}. For the grammar of the source query we used a modified
  grammar of the GSMC input language \cite{ACSI-D2.2.3}, with
  extensions that allow to ``extract'' artifact identifiers and their
  value attributes, so as to link them to the ontology. For more
  detail about \systemName, please refer to \cite{ACSI-D2.4.2}.
%The extended
%  syntax is:
%
\begin{comment}
{\footnotesize{
\begin{equation*}
\begin{split}
  \expression ~::=&~ \constantGSM
  ~\mid~ \{\variableGSM./path/attributeID\}\ == \ ?\variableGSM \\
  ~\mid&~ \expression\ \aopGSM \ \expression
  ~\mid~ \expression\ \lopGSM \ \expression
  ~\mid~ \{\variableGSM./path/attributeID\} \\
  ~\mid&~ \textbf{GSM.isStageActive}('\variableGSM','stageID') \\
  ~\mid&~ \textbf{GSM.isMilestoneAchieved}('\variableGSM','milestoneID') \\
  ~\mid&~ \variableGSM.attributeID1 \mbox{ -$>$ }
  \textbf{exists}(attributeID2 = \expression) \\
%%\end{split}
%%\end{equation*}
%
%\todo{I'm a bit unsure with the red part}
%
%%\begin{equation*}
%%\begin{split}
  \formula ~::=&~  \expression
~\mid~(\formula)
~\mid~\formula\ \andGSM\ \formula
~\mid~\formula\ \orGSM\ \formula
~\mid~\notGSM\ \formula
~\mid~\existsGSM ('variable',\ 'artifactID')(\formula)\\
~\mid&~\forallGSM ('variable',\ 'artifactID')(\formula)
~\mid~\getGSM('variable',\ 'artifactID')(\formula)\\
\end{split}
\end{equation*}
}}
\end{comment}
%
%###########################################################################################
%###########################################################################################
\end{inparaenum}
\begin{comment}
The two key additional features rely in the possibility of introducing
a variable assigning it to an expression (see the second line in the
grammar definition), and the possibility of ``getting'' a variable
representing an instance of the specified artifact (see the last line
in the grammar definition). These variables are considered to be free
in the specified query, and can be consequently used to ``transport''
values and artifact identifiers into the Semantic Layer, respectively
as attributes and object terms.
\end{comment}



































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% EXPLANATION ABOUT OBGSM MAIN COMPONENTS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}

\systemName\ \todo{I think this OBGSM components explanation can be
  omitted whenever needed} consists of the following main components:
%
\begin{inparaenum}[\it (i)]
%
\item \emph{Temporal Property Parser and Validator}. This component
  parses and validates a conceptual temporal property, checking its
  well-formedness and whether it guarantees the required restrictions
  or not. The parser for the temporal part of the property is implemented using Antlr 4.0  \footnote{\url{http://www.antlr.org}}. For parsing the local queries
  in the  temporal property, the \sparql parser component from
  \marianoSystem\ is extensively used, together with the \Jena library\footnote{\url{http://jena.apache.org}}.
  % We use the \Jena library mostly to restrict the \sparql query
  % fragment that we consider.
%
\item \emph{Ontology Parser}. This component, entirely provided by
  \marianoSystem, reads and parse an OWL 2 QL ontology.
%
\item \emph{Mapping Parser}. This component
  reads and parses the file containing mapping assertions. As for the
  implementation, the parser already present in \marianoSystem\ is
  reused and complemented with the additional features by using Antlr 4.0.
%
\item \emph{Temporal Property Rewriter}. When the input temporal
  property and the input ontology have been parsed, \systemName\ \emph{rewrites} the
  parsed temporal property based on the given ontology, using this component. The implementation of the
  query rewriting functionality is fully inherited from  \marianoSystem.
%
\item \emph{Unfolder}. This component takes the specification of
  mapping assertions and the property produced by the rewriter,
  producing the final unfolded property. To do so, it extends the base
  unfolding functionality already present in \marianoSystem.
%
\end{inparaenum}

\end{comment}


\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> submitted/5.1-GSM.tex <==
In this section, we show how the formal framework of $\sgds$s can be concretely instantiated, in the case where the transition relation at the Relational Layer is obtained from artifacts specified using the Guard-Stage-Milestone (GSM) approach. In particular, we show how existing techniques and tools have been suitably combined into a tool, called  \emph{\systemName}, which enables the verification of GSM-based artifacts with a Semantic Layer.

% We now concretize the formal framework described in Section \ref{sec:sas} by relying on Guard-Stage-Milestone (GSM) approach for Artifact Layer modeling, recently proposed by IBM \cite{Damaggio:2011:EIF:2040283.2040315} and included by the Object Management Group (OMG) into the new standard for Case Management Model and Notation (CMMN) \cite{cmmn:standard2013}. 
%

\smallskip
\noindent
\textbf{GSM Overview.}
For the sake of space, here we provide a general overview of the GSM
methodology and we refer to \cite{HDDF*11,DaHV13} for more detailed and formal
definitions.  GSM is a declarative modeling framework that has been designed to
simplify design and maintenance of business models.  The GSM information model
uses (possibly nested) attribute/value pairs to capture the domain of interest.
The key elements of a lifecycle model are \emph{stages}, \emph{milestones} and
\emph{guards} (see Figure~\ref{fig:claimingstage}).  Stages (represented as
rounded rectangles) are possibly hierarchical clusters of activities, intended
to update and extend the data of the information model. They are associated to
milestones (circles), business operational objectives which can be achieved
while the stage is under execution. Each stage has one or more guards
(diamonds), which control the activation of stages and, like milestones, are
described in terms of data-aware expressions, involving conditions over the
artifact information model.


\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/6-caseStudy.tex <==
\section{Case Study: Energy Scenario}
\label{sec:caseStudy}

%\todo[inline]{\textbf{TODO:} \\
%- Describe the use case in general and our specific domain of interest \\
%- Explain the GSM Model for this use case \\
%- Explain the semantic layer for this use case (explain the ontology
%and the mappings) \\
%- Explain the verification of some temporal property examples
%}

As a case study to demonstrate our approach we refer to the fragment of the
Energy Use Case Scenario developed within the ACSI Project \cite{ACSI-D5.5}.
We show how the Semantic Layer can be exploited in order to facilitate the
specification of temporal properties of interest, and discuss how these are
automatically translated into properties that can be directly verified by GSMC
over the Energy GSM model.
% We test \systemName\ to the Energy scenario which is inspired \todo{Should we
% say ``inspired'' or just say that it is a fragment of the ACSI Energy use
% case} by a fragment of the ACSI Energy use case\todo{reference to ACSI energy
% use case?}.

% \subsection{Energy Scenario at a Glance}\label{sec:EnergyUsecaseScenario}
\smallskip
\noindent
\textbf{Energy Scenario at a Glance.}
%
% For the sake of simplicity, in this section
We sketch the main aspects of the Energy Use Case, and refer
% the interested reader
to \cite{ACSI-D5.5} for further details.
%
% The Energy
This use case focuses on the electricity supply exchange process between
electric companies inside a distribution network.
% in Spain.
The
% electricity
exchange
% between companies
occurs at \emph{control points} (CP). Within a CP, a measurement of electricity
supply exchange takes place in order to calculate the fair remuneration that
the participating companies in the CP should receive. The measurement is done
by a \emph{meter reader company}, which corresponds to one of the companies
pertaining to that particular CP. The measurement results from the CP are then
submitted to the \emph{system operator}, who is in charge of processing the
results and publishing a \emph{CP monthly report}.
% If a participating company has any objection concerning the published
% measurement, the company can raise an objection.
A participating company can raise an objection concerning the published
measurement.  Once all the risen objections are resolved, the report is
closed. The collection of CP monthly reports is then represented as a \emph{CP
 monthly report accumulator}.

In order to implement the sketched scenario using the GSM methodology, we model
the \emph{Control Point Monthly Report $($CPMR$)$} as an artifact which
contains the information about hourly measurements done in a particular CP
within a certain month.  The lifecycle of an instance of this artifact begins
once the hourly measurements are provided, and runs until the liquidation for
the CP measurements has started. The artifact lifecycle consists of three root
stages:
\begin{inparaenum}[\it (i)]
\item \emph{CPMRInitialization}, which is activated when a new instance of the
  CPMR artifact is created.
\item \emph{Claiming}, which handles the submission of measurements, and the
  subsequent reviewing procedure during which objections may be raised.
\item \emph{MeasurementUpdating}, which is activated once an event is raised,
  requesting for updating the measurement results.
\end{inparaenum}

Figure~\ref{fig:GSM Model} shows a GSM model of the \emph{Claiming} stage, on
which we focus here.  It contains the following five sub-stages:
\begin{inparaenum}[\it (i)]
\item \emph{Drafting}, which models the process of submitting and processing
  the CP hourly measurements and processing a draft of the CPMR.
\item \emph{Evaluating}, which is responsible for official measurement
  publication.
\item \emph{Reviewing}, which models the process of either accepting the
  official measurement, or deciding whether the difference is acceptable or
  not. Such decision may result in an objection either by the Metering Office
  (MO) or the Energy Control Department (ECD).
\item \emph{CreateObjection}, which corresponds to creation of a new Objection
  instance.
\item \emph{Closing}, which is responsible for closing the objection
  period. Once this period finishes and there are no requested objections, the
  monthly report is finalized and the \emph{CPMRFinished} milestone is
  achieved.
\end{inparaenum}
The collection of CP monthly reports for a specific month is then modeled by
the \emph{CPMR Monthly Accumulator $($CPMRMA$)$} artifact.

\begin{figure}[btp]
  \label{fig:claimingstage}
  \centering
  \includegraphics[width=\textwidth]{GSMModelForCPMRClaimingStage_cut}
  \caption{The Claiming Stage in the GSM Model for the CPMR Artifact}
  \label{fig:GSM Model}
\end{figure}

\smallskip
\noindent
\textbf{The Semantic Layer for the Energy Use Case.}
% \subsection{The Semantic Layer for the ACSI Energy Use
% Case}\label{sec:EnergyUsecaseSemanticLayer}
Here we provide a Semantic Layer built on top of the GSM model for the Energy
scenario, restricting our attention to the Control Point
Measurement Report (CPMR).

\smallskip
\noindent
\textbf{The Ontology TBox.}  We consider the following states of a control
point measurement report:
\begin{inparaenum}[\it (i)]
\item a finished CPMR (when the milestone \emph{CPMRFinished} is achieved),
\item a reviewed CPMR (after finishing the review inside the \emph{Reviewing}
  stage)
\item an accepted CPMR (when the milestone \emph{PublishedOK} is achieved)
\item an objected CPMR.
\end{inparaenum}
%
Following this intuition, a portion of the ontology TBox of the Semantic Layer
is depicted in Figure~\ref{fig:EnergyOntology}, together with its
representation as a UML Class Diagram.
%
% An UML model for the ontology of the Semantic Layer is depicted in
% Figure~\ref{fig:EnergyOntology}.

\begin{figure}[btp]
  %\centering
  \raisebox{-0.6cm}{\includegraphics[width=0.6\textwidth]{EnergyOntology4}}
  %
  \makebox[1cm][l]{\scriptsize
   $
   \begin{array}{rl}
     \SOMET{\mathit{contains}} &\ISA \mathit{PublishedCPReportColl.}\\
     \SOMET{\INV{\mathit{contains}}} &\ISA \mathit{PublishedCPReport} \\
     \SOMET{\mathit{controlPointID}} &\ISA \mathit{PublishedCPReport}\\
     \SOMET{\INV{\mathit{controlPointID}}} &\ISA \mathit{String}\\
     \mathit{FinishedReport} &\ISA \mathit{PublishedCPReport}\\
     &\cdots\\
     %\mathit{ReviewedReport} &\ISA \mathit{PublishedCPReport}\\
     %\mathit{AcceptedReport} &\ISA \mathit{PublishedCPReport}\\
     %\mathit{ObjectedReport} &\ISA \mathit{PublishedCPReport}
   \end{array}
   $}

  \caption{Ontology for the CPMR reviewing process in the Energy scenario}
  \label{fig:EnergyOntology}
  \vspace{-5mm}
\end{figure}

\smallskip
\noindent
\textbf{The Mapping Assertions.}
%
% We use the following mapping assertions in order to link the
% information model in the GSM model to the Semantic Layer. The
% assertions are written in the mapping specification language of
% \systemName.
%
We use mapping assertions as described in Section~\ref{sec:obgsmtool} in order
to link the GSM information model to the Semantic Layer. Due to the space limitations, we
only give an example of such a mapping in the \systemName mapping specification
language:

\begin{comment}
\noindent {\tt \scriptsize{%
mappingId \hspace*{1 mm} ReviewedReportMapping \\
target \hspace*{5 mm} <"\&:;cpmr/\{\$x\}/"> rdf:type :ReviewedReport . \\
source \hspace*{5 mm} get('x','CPMR')(GSM.isMilestoneAchieved('x','AcceptingPublishedOK') OR \\
\hspace*{25 mm} GSM.isMilestoneAchieved('x','MOReviewingPublishedOK') OR \\
\hspace*{25 mm}
GSM.isMilestoneAchieved('x','ECDReviewingPublishedOK'))\\
\textrm{\normalsize where ``:'' is a prefix declared as
 {\tt\footnotesize http://acsi/example/energy/energy.owl\#}.\\}
}}
\end{comment}

{\scriptsize
\begin{verbatim}
 mappingId  ReviewedReportMapping
 target     <"&:;cpmr/{$x}/"> rdf:type :ReviewedReport .
 source     get('x','CPMR')(GSM.isMilestoneAchieved('x','AcceptingPublishedOK') OR
                       GSM.isMilestoneAchieved('x','MOReviewingPublishedOK') OR
                       GSM.isMilestoneAchieved('x','ECDReviewingPublishedOK'))
\end{verbatim}
}%
\noindent
% where ``:'' is a prefix declared as {\tt\footnotesize
% http://acsi/example/energy/energy.owl\#}.
%
Intuitively, this mapping populates the $\mathit{ReviewedReport}$ concept with
the CPMR artifact instances, given the achievement of either of the milestones:
\emph{AcceptingPublishedOK}, \emph{MOReviewingPublishedOK}, or
\emph{ECDReviewingPublishedOK}. In the Semantic Layer,
$\mathit{ReviewedReport}$ intuitively represents a CPMR that has been
reviewed. In the Artifact Layer, this corresponds to the situation in which the
CPMR has been reviewed and accepted either by the electric company, or by the
metering office (MO), or by the Electric Control Department (ECD). This example
shows how such details can be abstracted away in the Semantic Layer, which does
not show that a $\mathit{ReviewedReport}$ is obtained by a (possibly complex)
chaining of achieved milestones in the underlying GSM model.

%%%%%%%%%%%%%% Removed by Babak because of space issues

% Another example of mapping assertion, which intuitively populates the
% $contains$ role by relating CPMRMA with the CPMRs it contains is as
% follows:

% {\scriptsize
% \begin{verbatim}
%  mappingId  CPMRMAContainsCPRMMapping
%  target     <"&:;cpmrma/{$x}/"> :contains <"&:;cpmr/{$y}/"> .
%  source     get('x','CPMRMA')(get('y','CPMR')(
%                          x./CPMRMA/CPMRDATA->exists(CPMRID == {y./CPMR/ID})))
% \end{verbatim}
% }

\smallskip
\noindent
\textbf{Verification within the Energy Use Case.}
% \subsection{Verification within the ACSI Energy Use
% Case}\label{sec:ExperimentEnergyVerification}
We demonstrate now how the presence of the Semantic Layer may help when
specifying different temporal properties of interest.  For example, consider a
property saying that: \emph{``All control point monthly reports will eventually
 be finished''}.  This can be expressed as a conceptual temporal property over
the Semantic Layer defined above:
\[
  \AG (\forallTemp\ x.\ ([\mathit{PublishedCPReport}(x)] \implTempB \EF
  [\mathit{FinishedReport}(x)]) )
\]
Then it can be encoded in the machine-readable SPARQL-based verification
language, defined in Section \ref{sec:obgsmtool}, as follows:

%{\tt \fontsize{7.7}{7.7}\selectfont
%\hspace*{0.5mm} AG (FORALL ?x.([PREFIX : <http://acsi/example/ACSIEnergy/ACSIEnergy.owl\#> \\
%\hspace*{25.5mm} SELECT ?x WHERE { ?x a :ControlPointReport}] -> \\
%\hspace*{19mm} EF [PREFIX : <http://acsi/example/ACSIEnergy/ACSIEnergy.owl\#> \\
%\hspace*{25.5mm} SELECT ?x WHERE { ?x a :FinishedReport}] \\
%\hspace*{15mm} ));
%}%
%
{\fontsize{7.7}{7.7}\selectfont
\begin{verbatim}
AG (FORALL ?x.([PREFIX : <http://acsi/example/ACSIEnergy/ACSIEnergy.owl#>
                SELECT ?x WHERE { ?x a :PublishedCPReport}] ->
            EF [PREFIX : <http://acsi/example/ACSIEnergy/ACSIEnergy.owl#>
                SELECT ?x WHERE { ?x a :FinishedReport}]
          ));
\end{verbatim}
}

We now show how this kind of high-level properties are processed by \systemName
into temporal properties formulated over the GSM model and which can be fed to
the GSMC model checker.  Notice that without the Semantic Layer and
\systemName, the user would have to construct the low-level properties
manually.

We first perform a rewriting step, which expands concepts contained in the
property of interest using the ontology TBox. In our example, this results in
the conceptual property
%
$\AG (\text{PCR}(x) \implTempB \EF [\mathit{FinishedReport}(x)]))$,
%
in which:
%{\footnotesize
\[
  \text{PCR}(x) =
  \begin{array}[t]{@{}l}
    \existsTemp\ y\ .\
    [\mathit{hasControlPointID}(x,y)] \orTempB
    [\mathit{ObjectedReport}(x)] \orTempB \\{}
    [\mathit{AcceptedReport}(x)] \orTempB
    [\mathit{PublishedCPReport}(x)] \orTempB
    [\mathit{ReviewedReport}(x)] \\{}
    \orTempB [\mathit{FinishedReport}(x)] \orTempB
    (\existsTemp\ z\ .\ [\mathit{contains}(z,x)])
  \end{array}
\]
%}%
% The example of the rewriting steps result above exhibit the reasoning
% capability done by \systemName in order to take into account the knowledge
% encoded in the ontology within the verification.
In particular, the rewriting step employs reasoning over the \dlliter TBox by
taking into account the following knowledge contained in the Semantic Layer:
%
\begin{inparaenum}[\it (i)]
\item Those objects that have a control point ID (i.e., are in the domain of the
  attribute $\mathit{hasControlPointID}$), are instances of
  $\mathit{PublishedCPReport}$;
\item $\mathit{ObjectedReport}$ is a $\mathit{PublishedCPReport}$;
\item $\mathit{AcceptedReport}$ is a $\mathit{PublishedCPReport}$;
\item $\mathit{ReviewedReport}$ is a $\mathit{PublishedCPReport}$;
\item Those objects that are in the range of the role $contains$ are
  instances of $\mathit{PublishedCPReport}$;
\item $\mathit{FinishedReport}$ is a $\mathit{PublishedCPReport}$.
\end{inparaenum}


\begin{figure}[tp]
  \centering
  \footnotesize
\[
  % AG (  forall( 'x33', 'CPMR' )( !  (
  \AG\ ( \forallGSM ('x',
  \begin{array}[t]{@{}l}
    \ '\mathit{CPMR}')(!(\GSMisMSachieved('x','\mathit{Objected}') \orTempB\\
    % \GSMisMSachieved('x33','Objected') ||
    \GSMisMSachieved('x','\mathit{ObjectionRequested}')  \orTempB\\
    % \GSMisMSachieved('x33','\mathit{ObjectionRequested}')  ||
    \GSMisMSachieved('x','\mathit{ObjectionCreated}') \orTempB\\
    % \GSMisMSachieved('x33','\mathit{ObjectionCreated}') ||
    \GSMisMSachieved('x','\mathit{MOReviewingObjectionRequested}') \orTempB\\
    % \GSMisMSachieved('x33','\mathit{MOReviewingObjectionRequested}')  ||
    \GSMisMSachieved('x','\mathit{ECDReviewingObjectionRequested}')   \orTempB\\
    % \GSMisMSachieved('x33','\mathit{ECDReviewingObjectionRequested}')   ||
    \GSMisMSachieved('x','\mathit{PublishedOK}') \orTempB\\
    % \GSMisMSachieved('x33','\mathit{PublishedOK}') ||
    % ( false ) \orTempB\\
    % ( true ) ||\\
    \GSMisMSachieved('x','\mathit{AcceptingPublishedOK}') \orTempB\\
    % \GSMisMSachieved('x33','\mathit{AcceptingPublishedOK}') ||
    \GSMisMSachieved('x','\mathit{MOReviewingPublishedOK}') \orTempB\\
    % \GSMisMSachieved('x33','\mathit{MOReviewingPublishedOK}') ||
    \GSMisMSachieved('x','\mathit{ECDReviewingPublishedOK}') \orTempB\\
%\GSMisMSachieved('x33','\mathit{ECDReviewingPublishedOK}') ||
    \existsGSM( 'y', '\mathit{CPMRMA}' )  ( y./\mathit{CPMRMA}/\mathit{CPMRDATA} \implTempB \\
    \hspace{2cm}\textbf{exists}(\mathit{CPMRID} == {x./\mathit{CPMR}/\mathit{ID}}) )  \orTempB\\
    % exists('x34', '\mathit{CPMRMA}') (x34./CPMRA/CPMRDATA->exists(CPMRID == {x33./CPMR/ID}) )  ||
    \GSMisMSachieved('x','\mathit{CPMRFinished}')) \orTempB\\
    % \GSMisMSachieved('x33','\mathit{CPMRFinished}'))   ||
    EF  ( \GSMisMSachieved('x','\mathit{CPMRFinished}'))))\\
    % EF  ( \GSMisMSachieved('x33','\mathit{CPMRFinished}'))))
  \end{array}
\]
  \vspace{-5mm}
  \caption{Resulting temporal property over the GSM model}
  \label{fig:example-property}
  \vspace{-3mm}
\end{figure}

%Notice that the absence of a mapping assertion for the concept
%$ControlPointReport$ results into a $false$ disjunct in the unfolding.

We then perform the unfolding step, which exploits the mapping assertions in
order to reformulate the rewritten property to the temporal property over the
GSM model.
%
Such property, shown in Figure~\ref{fig:example-property}, can be now be fed to
the GSMC model checker in order to validate the initial property claiming that
\emph{``all control point monthly reports will eventually be finished''}.
Given the significant difference in complexity between the property formulation
over the Semantic Layer and its corresponding translation over GSM, the
advantage of the presence of the Semantic Layer becomes apparent even for this
simple case study.  Conceptual temporal property formulation allows to hide
low-level details from the user and enables the modeler to rather focus on the
domain under study using the vocabulary he/she is familiar with.

%  see from the examples above that the existence of semantic
% layer simplified the way how we can express the property that we want
% to verify. Not only on the compactness of the property that we need to
% write, the presence of semantic layer also ease us to specify the
% temporal property by abstracting away many low level details,
% additionally it provides the intuitive vocabularies based on our
% domain interest.



\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/7-discussion-old.tex <==
\section{Discussion and Conclusion}
\label{sec:discussion}


% In this paper we propose a framework for modeling artifact systems
% using novel expressive languages for artifact-centric systems such as
% GSM, which provides domain independent conceptual view of the system
% expressed using OWL 2 QL, and connected to the original system using
% mapping specifications. The ontology provides a high-level
% understanding of the system, which can be exploited to verify the
% correct behavior of the system. The queries and the properties to be
% verified over such system are expressed over the vocabulary of the
% high-level semantic layer, and using the provided techniques and tool
% will be translated to queries over the low-level artifact system.

% In this paper we propose a framework for modeling artifact systems,
% and connecting the models to a domain independent conceptual view of
% the system expressed as an OWL 2 QL ontology. 
%%
In this paper we introduce a technique for rewriting (temporal)
queries expressed in the vocabulary of a given semantic layer, to
temporal properties over the database layer of the system based on the
mappings between the database and the semantic layer. 

The technique based on rewriting of the queries can also be applied to
verify the artifact system based on model checking of the temporal
properties over the vocabulary of the semantic layer, provided that
all of the states of the artifact-artifact system are consistent with
the semantic layer. In this technique, the queries over the semantic
layer are rewritten based on the ontology, and then the problem to
model checking of resulting queries is delegated to existing model
checkers such as GSMC, considering them as a black box.  In the
example of Section \ref{sec:caseStudy}, the TBox does not contain any
disjointness axiom, and consequently, all the states of the artifact
system are consistent w.r.t. the TBox, and we can apply the mentioned
technique to verify the system.

However, in general, the consistency of the states of the artifact and
the conceptual level are not guaranteed. In such a situation the
strategy followed in this paper based on delegating the verification
of \ctla properties to the existing model checkers cannot
be followed. One possible solution is to provide a mechanism for the
model checkers to exploit the ontology of the conceptual level to
distinguish the consistent and inconstant states of the low-level
system. The other possible solution is to consider less expressive
temporal logics, i.e., fragments of \ctla. These latter scenarios
have not been addressed in this paper, and provide us with 
interesting problems for future investigations.

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/7-discussion.tex <==
\section{Discussion and Conclusion}
\label{sec:discussion}


% In this paper we propose a framework for modeling artifact systems
% using novel expressive languages for artifact-centric systems such as
% GSM, which provides domain independent conceptual view of the system
% expressed using OWL 2 QL, and connected to the original system using
% mapping specifications. The ontology provides a high-level
% understanding of the system, which can be exploited to verify the
% correct behavior of the system. The queries and the properties to be
% verified over such system are expressed over the vocabulary of the
% high-level semantic layer, and using the provided techniques and tool
% will be translated to queries over the low-level artifact system.

% In this paper we propose a framework for modeling artifact systems, and
% connecting the models to a domain independent conceptual view of the system
% expressed as an OWL 2 QL ontology.
%%
In this paper we have introduced a framework in which an artifact system based
on the GSM model is connected through declarative mappings to a Semantic Layer
expressed as an OWL~2~QL ontology, and temporal properties expressed over the
Semantic Layer are reformulated in terms of the underlying GSM model and
verified over its execution, using state of the art OBDA and model checking
technology.
%
We have assumed in our development
% that all states generated by the execution of the artifact system are
% consistent with the Semantic Layer.  Indeed, such states are not directly
% accessible during verification, given that they are generated by the GSMC
% model checker, which we use as a black box.
that all states generated for the purpose of verification by the GSMC model
checker (which we use as a black box), are consistent with the Semantic Layer.
Indeed, inconsistent states could not be easily pruned away, as e.g., the
approach proposed in \cite{CDLMS12} would require.
%
Notice that in our case study presented in Section~\ref{sec:caseStudy} such
assumption holds since the TBox does not contain any disjointness assertions.
% and consequently the underlying artifact system cannot generate states that
% are inconsistent w.r.t.\ the TBox,

However, in general, the consistency of the states at the artifact level with
the TBox in the Semantic Layer is not guaranteed.  In such a situation the
strategy proposed here, based on delegating the verification of \ctla
properties to the existing model checker, cannot be followed directly.  One
possible solution to this is to provide a mechanism for the model checker to
exploit the ontology at the Semantic Layer to distinguish consistent from
inconsistent states of the low-level system.  The other possible solution is to
consider less expressive temporal logics, i.e., fragments of \ctla, and
investigate whether the check for consistency can be embedded in the formula to
verify.  These latter scenarios provide us with interesting problems for future
investigation.

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/8-conclusion.tex <==
% \section{Conclusion}
% \label{sec:conclusion}


% \endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> submitted/macros-specific.tex <==
\newcommand{\statew}{1.2 cm}
\newcommand{\stateh}{1.2 cm}
\newcommand{\displx}{1.7 cm}
\newcommand{\disply}{1.5 cm}

\newcommand{\actions}{\ensuremath{\mathit{actions}}}

\newcommand{\AAAM}{\ensuremath{A^3M}\xspace}

%------------------------------------------------------------- Domain
\newcommand{\const}[1]{\C_{#1}}

\newcommand{\CONST}{\C}

\newcommand{\FUNC}{\ensuremath{\F}\xspace}   % Set of function names
\newcommand{\HERBAND}{\HERBRAND}
\newcommand{\HERBRAND}{\ensuremath{\mathbb{U}}\xspace}
 % Herbrand universe
\newcommand{\PART}[1]{\ensuremath{P^{#1}}}   % Partitioning of a given set

%------------------------------------------- Data Layer
\newcommand{\dl}{\ensuremath{\D}\xspace}
\newcommand{\schema}{\ensuremath{\R}\xspace}
\newcommand{\DBschema}{\schema}
%\newcommand{\schema}{\bsy{R}}
\newcommand{\idb}{\ensuremath{\I_0}\xspace}
%------------------------------------------- Process Layer
\newcommand{\pl}{\ensuremath{\P}\xspace}
\newcommand{\aset}{\ensuremath{\A}\xspace}
\newcommand{\rset}{\ensuremath{\varrho}\xspace}
\newcommand{\pos}[1]{\ensuremath{#1^+}\xspace}

\newcommand{\sys}{\ensuremath{\S}\xspace}
\newcommand{\dcds}{\mbox{DCDS}\xspace}
\newcommand{\rexec}[1]{\textsc{exec}_{#1}\xspace}
\newcommand{\sexec}[1]{\textsc{a-exec}_{#1}\xspace}

\newcommand{\kbds}{\mbox{KBDS}\xspace}

\newcommand{\KA}{\mathcal{KA}}
 \newcommand{\kabm}{\mathcal{M}}
\newcommand{\kabv}{\Delta}
\newcommand{\kabtbox}{\mathcal{T}}
\newcommand{\kabkb}{\mathcal{K}}
\newcommand{\kabaction}{\Gamma}
\newcommand{\kababox}{\mathcal{A}}



%-------------------------------------------------------
% SGDS stuff
%-------------------------------------------------------
\newcommand{\sgds}{\mbox{SAS}\xspace}
\newcommand{\sgdsSym}{\ensuremath{\S}\xspace}
\newcommand{\sgdsTup}{\tup{\obdaSym, \procCompSym, \DBinit}}

%Database
\newcommand{\DB}{\D}
\newcommand{\DBinst}{\I}
\newcommand{\DBinit}{\idb} %initial DB
\newcommand{\VALUE}{\V}
\newcommand{\Instances}{\Gamma}


\newcommand{\rws}{\rightsquigarrow}
\newcommand{\mapping}{\M}
%OBDA System
\newcommand{\obda}{\mbox{OBDA}\xspace}
\newcommand{\obdaSym}{\ensuremath{\O}\xspace}
\newcommand{\obdaTup}{\tup{\DBschema, \TBox, \mapping}}

%Rewriting
%\newcommand{\rew}{}

%Unfolding
\newcommand{\unfoldSig}{{\textsc{unfold}()}}
\newcommand{\unfold}[2]{{\textsc{unfold}(#1,#2)}}
\newcommand{\ucqunfoldSig}{\textsc{UCQ-unfold}}
\newcommand{\ucqunfold}[2]{\ucqunfoldSig(#1,#2)}
\newcommand{\eqlUnfoldSig}{{\textsc{EQL-unfold}()}}
\newcommand{\eqlUnfold}[2]{{\textsc{EQL-unfold}(#1,#2)}}
\newcommand{\skoTermSet}{sk(\mapping)}
\newcommand{\qunsat}[1]{\ensuremath{\mathsf{q}_\mathsf{unsat}(#1)}}
\newcommand{\TSd}{\Upsilon_{\dcdsSym}^{\scriptsize{\text{DCDS}}}}
\newcommand{\skolem}{\textsc{fs}}


%-------------------------------------------------------
% Transition System stuff
%-------------------------------------------------------
%Transition System in Relational Layer
\newcommand{\TSAs}{\Sigma}
\newcommand{\TSAt}{\Rightarrow}
\newcommand{\TSAsym}{\Upsilon^{\scriptsize{\text{R}}}} %\newcommand{\TStup}{\tup{\Delta,\R,\Sigma,s_0,\abox,{\Rightarrow}}}
\newcommand{\TSAtup}{\tup{\R, \TSAs, s_0, \db, \TSAt}}
\newcommand{\TBox}{\T}
\newcommand{\ABox}{A}

%Transition System in Semantic Layer
\newcommand{\TSSs}{\Sigma}
\newcommand{\TSSt}{\Rightarrow}
\newcommand{\TSSsym}{\Upsilon^{\scriptsize{\text{S}}}} %\newcommand{\TStup}{\tup{\Delta,\R,\Sigma,s_0,\abox,{\Rightarrow}}}
\newcommand{\TSStup}{\tup{\TBox, \TSSs, s_0, \abox, \TSSt}}



%------------------------------------------- Properties

\newcommand{\mulg}{\mulgq}
\newcommand{\muladom}{\ensuremath{\muL_{A}}\xspace}
\newcommand{\muladomEQL}{\ensuremath{\muL_{A}^{EQL}}\xspace}
\newcommand{\ctla}{ \textnormal{CTL}\ensuremath{_A}\xspace}

\newcommand{\mulpers}{\ensuremath{\muL_{P}}\xspace}
\newcommand{\hmadom}{\ensuremath{\L_{A}}\xspace}
\newcommand{\hmpers}{\ensuremath{\L_{P}}\xspace}
\newcommand{\muladl}{\ensuremath{\muladom^{{\textnormal{EQL}}}}\xspace}
\newcommand{\mulpdl}{\ensuremath{\mulpers^{{\textnormal{EQL}}}}\xspace}
\newcommand{\ctladl}{\ensuremath{\ctla^{{\textnormal{EQL}}}}\xspace}


\newcommand{\hbsim}{\approx}
\newcommand{\pbsim}{\sim}

\newcommand{\inadom}{\ensuremath{\textsc{live}}}

\newcommand{\restrict}[2]{\ensuremath{#1 \vert_{#2}}}

\newcommand{\prop}[1]{\ensuremath{\textsc{prop}(#1)}}


\newcommand{\muL}{\mu\L} % MuL - modal mu calculus - language
\newcommand{\muLclosed}{\muL_{C}}
\newcommand{\muLinitialdomain}{\muL_{{\I_0}}}
\newcommand{\muLguarded}{\muL_{G}}
\newcommand{\hmLguarded}{\L_{G}}
\newcommand{\muLglobal}{\muL_{\forall\exists G}}
%\newcommand{\muLglobal}{\muL_{(\forall,\exists)^*G}}

%------------------------------------------- Artifact System Syntax

\newcommand{\rmap}{\ensuremath{\M}\xspace}
\newcommand{\rmapext}{\ensuremath{\widehat{\M}}\xspace}

\newcommand{\rmapec}{\ensuremath{\rmap}}
   % Interpretation  of skolem terms
\newcommand{\terms}[1]{\textsc{terms}(#1)} % terms used in a given
                                % partitioning
\newcommand{\subterms}{\textsc{subTerms}}
\newcommand{\EC}{\ensuremath{\E}}       % Set of equality constraints
\newcommand{\ec}{\textit{ec}}          % An equality constraint.
\newcommand{\history}{\ensuremath{\H}} % History of a artifact system
                                % instance

% _________

%----------------------------------------------------------------
\newcommand{\VDO}[4]{\mbox{DO}^V\big(#1,\ #2,\ #3,\ #4\big)}
\newcommand{\RDO}[3]{\mbox{DO}^R\big(#1,\ #2,\ #3\big)}
\newcommand{\SDO}[3]{\mbox{DO}^S\big(#1,\ #2,\ #3\big)}

\newcommand{\VCLOSURE}[3]{\mbox{CLOSURE}^V\big(#1,\ #2,\ #3\big)}
\newcommand{\RCLOSURE}[3]{\mbox{CLOSURE}^R\big(#1,\ #2,\ #3\big)}
\newcommand{\SCLOSURE}[3]{\mbox{CLOSURE}^S\big(#1,\ #2,\ #3\big)}

\newcommand{\VEXECUTE}[3]{\mbox{EXECUTE}_{closed}^V\big(\tup{#1,#2},\ #3\big)}
\newcommand{\REXECUTE}[3]{\mbox{EXECUTE}_{closed}^ R\big(\tup{#1,#2},\ #3\big)}
\newcommand{\SEXECUTE}[3]{\mbox{EXECUTE}_{closed}^S\big(\tup{#1,#2},\ #3\big)}

%-----------------------------------------------------------------

% Next generations of Do, Closure, and Execute:

\newcommand{\doo}[3]{\textsc{do}^{#1}_{#2}(#3)}
\newcommand{\effect}[1]{\textsc{effect}(#1)}
% \do { S | R | V }{CLOSE | OPEND | OPENN} { \I,\P, ... }

\newcommand{\closure}[3]{\textsc{closure}^{#1}_{#2}(#3)}
% \closure { S | R | V }{CLOSE | OPEND | OPENN} { \I,\P, ... }

\newcommand{\sexecute}[3]{\textcolor{red}{\textsc{s-}\execute{#1}{#2}{#3}}\xspace}
\newcommand{\rexecute}[3]{\textcolor{red}{\execute{#1}{#2}{#3}}\xspace}

\newcommand{\execute}[3]{\ensuremath{\textsc{execute}^{#1}_{#2}#3}\xspace}
% \execute { S | R | V }{CLOSE | OPEND | OPENN} { \I,\P, ... }
%------------------------------------------------------------------

\newcommand{\VEXECUTEO}[3]{\mbox{EXECUTE}_{open}^V\big(\tup{#1,#2},\ #3\big)}
\newcommand{\REXECUTEO}[3]{\mbox{EXECUTE}_{open}^R\big(\tup{#1,#2},\ #3\big)}
\newcommand{\SEXECUTEO}[3]{\mbox{EXECUTE}_{open}^S\big(\tup{#1,#2},\ #3\big)}

\newcommand{\RDOC}{\mbox{DO}^R}
\newcommand{\SDOC}{\mbox{DO}^S}

\newcommand{\REXTRC}{\mbox{EXTRACT\_CALLS}}
\newcommand{\REXTRCL}{\mbox{EXTRACT\_CLASSES}}
\newcommand{\RCALLC}{\textsc{serviceCalls}}
\newcommand{\RCOMM}{\textsc{pickCommitment}}
\newcommand{\pickVal}{\textsc{pickValue}}
\newcommand{\callService}{\textsc{callService}}


%-------------------------------------------------- Macros of the example
%--- NonDet Schema
\newcommand{\eSysStatus}{\ensuremath{\mathsf{Status}}\xspace}
\newcommand{\eApplicant}{\ensuremath{\mathsf{Applicant}}\xspace}
\newcommand{\eTravel}{\ensuremath{\mathsf{Travel}}\xspace}
\newcommand{\eHotel}{\ensuremath{\mathsf{Hotel}}\xspace}
\newcommand{\eFlight}{\ensuremath{\mathsf{Flight}}\xspace}
\newcommand{\eTrStatus}{\ensuremath{\mathsf{Status}}\xspace}
\newcommand{\eTrue}{\ensuremath{\mathsf{True}\xspace}\xspace}

\newcommand{\eTravelA}{\ensuremath{\mathsf{Travel$_A$}}\xspace}
\newcommand{\eHotelA}{\ensuremath{\mathsf{Hotel$_A$}}\xspace}
\newcommand{\eFlightA}{\ensuremath{\mathsf{Flight$_A$}}\xspace}

\newcommand{\eToPay}{\ensuremath{\mathsf{ToPay}}\xspace}
\newcommand{\eReject}{\ensuremath{\mathsf{Rejected}}\xspace}

%--- Attributes
\newcommand{\eId}{\ensuremath{\mathsf{id}}\xspace}
\newcommand{\eClientName}{\ensuremath{\mathsf{eName}}\xspace}
\newcommand{\eHotelName}{\ensuremath{\mathsf{hName}}\xspace}
\newcommand{\ePosition}{\ensuremath{\mathsf{position}}\xspace}
\newcommand{\eTrId}{\ensuremath{\mathsf{trId}}\xspace}
\newcommand{\eDate}{\ensuremath{\mathsf{date}}\xspace}
\newcommand{\eStatus}{\ensuremath{\mathsf{status}}\xspace}
\newcommand{\eLocation}{\ensuremath{\mathsf{location}}\xspace}
\newcommand{\eReason}{\ensuremath{\mathsf{reason}}\xspace}
\newcommand{\ePrice}{\ensuremath{\mathsf{price}}\xspace}
\newcommand{\eCurrency}{\ensuremath{\mathsf{currency}}\xspace}
\newcommand{\eUSDPrice}{\ensuremath{\mathsf{priceInUSD}}\xspace}
\newcommand{\eCurrencyRate}{\ensuremath{\mathsf{currencyRate}}\xspace}
\newcommand{\eVerifiedPrice}{\ensuremath{\mathsf{verifiedPrice}}\xspace}
\newcommand{\eVerifiedPriceInUSD}{\ensuremath{\mathsf{checkedPriceInUSD}}\xspace}
\newcommand{\ePhone}{\ensuremath{\mathsf{phone}}\xspace}
\newcommand{\eFNumber}{\ensuremath{\mathsf{fNum}}\xspace}
\newcommand{\eVerified}{\ensuremath{\mathsf{verified}}\xspace}
\newcommand{\eTrConfStatus}{\ensuremath{\mathsf{verificationStatus}}\xspace}
\newcommand{\eLiveAt}{\ensuremath{\mathsf{status}}\xspace}
\newcommand{\ePassed}{\ensuremath{\mathsf{passed}}\xspace}
%--- Values
\newcommand{\eRFR}{\textit{`readyForRequest'}}
\newcommand{\eRTV}{\textit{`readyToVerify'}}
\newcommand{\eRTU}{\textit{`readyToUpdate'}}
\newcommand{\eRC}{\textit{`requestConfirmed'}}

\newcommand{\eNV}{\ensuremath{\mathsf{notVerified}}\xspace}

%--- Det Values
\newcommand{\ePhaseC}{\textit{`checkPrice'}\xspace}
\newcommand{\ePhaseD}{\textit{`checkTravel'}\xspace}

\newcommand{\eVALPrice}{\textit{price}\xspace}

\newcommand{\eValVerified}{\ensuremath{\mathsf{verified}\xspace}}
\newcommand{\eValNotVerified}{\ensuremath{\mathsf{notVerified}\xspace}}

\newcommand{\eValChecked}{\textit{checked}\xspace}
\newcommand{\eValNotChecked}{\textit{notChecked}\xspace}

\newcommand{\eValPassed}{\textit{passed}\xspace}
\newcommand{\eValNotPassed}{\textit{notPassed}\xspace}

%--- Det Variables
\newcommand{\eVarPrice}{\mathit{price}\xspace}
\newcommand{\eVarCurrency}{\mathit{currency}\xspace}
\newcommand{\eVarCurrencyRate}{\mathit{currencyRate}\xspace}
\newcommand{\eVarDate}{\mathit{date}\xspace}
\newcommand{\eVarPriceInUSD}{\mathit{priceInUSD}\xspace}
%--- NonDeterministic Service Calls
\newcommand{\escTrId}{\textsc{genTrId}()\xspace}
\newcommand{\escClientName}{\textsc{inEName}() \xspace}
\newcommand{\escDate}{\textsc{inDate}() \xspace}
\newcommand{\escTrReason}{\textsc{inReason}() \xspace}
\newcommand{\escHName}{\textsc{inHName}() \xspace}
\newcommand{\escHDate}{\textsc{inHDate}() \xspace}
\newcommand{\escHPricec}{\textsc{inHPrice}() \xspace}
\newcommand{\escHCurrency}{\textsc{inHCurrency}() \xspace}
\newcommand{\escHPUSD}{\textsc{inHPInUSD}() \xspace}
\newcommand{\escFDate}{\textsc{inFDate}() \xspace}
\newcommand{\escFNumber}{\textsc{inFNum}() \xspace}
\newcommand{\escFprice}{\textsc{inFPrice}() \xspace}
\newcommand{\escFlightCurrency}{\textsc{inFCurrency}() \xspace}
\newcommand{\escFPUSD}{\textsc{inFPUSD}() \xspace}
\newcommand{\escVerifyTravel}[2]{\textsc{verifyTravel}(#1,#2) \xspace}
\newcommand{\escMakeDecision}[1]{\textsc{makeDecision}(#1) \xspace}



%-- my effect shortcut
 \newcommand{\rsa}{\rightsquigarrow}

%--- Deterministic Service Calls
\newcommand{\escGetCurrencyRate}[2]{\textsc{getCurrencyRate}(#1,#2)}
\newcommand{\escCalPriceInUSD}[2]{\textsc{calculatePriceInUSD}(#1,#2)}
\newcommand{\escComparePrice}[2]{\textsc{comparePrice}(#1,#2)}
\newcommand{\escConvertAndCheck}{\textsc{convertAndCheck}}
\newcommand{\escCheckPrice}{\textsc{comparePrice}}

%--- NonDet Actions
\newcommand{\eAReimburseRequest}{\textit{InitiateRequest}\xspace}
\newcommand{\ePriliminaryCheck}{\textit{VerifyRequest}\xspace}
\newcommand{\eUpdateRequest}{\textit{UpdateRequest}\xspace}
\newcommand{\eAcceptRequest}{\textit{AcceptRequest}\xspace}


%---Det Actions
\newcommand{\eGetCurrencyRate}{\textit{GetCurrencyRate}\xspace}
\newcommand{\eCalPriceInUSD}{\textit{CalculatePriceInUSD}\xspace}
\newcommand{\eCheckPrice}{\textit{CheckPrice}\xspace}
\newcommand{\eCheckTravel}{\textit{CheckTravel}\xspace}


%-----------------------------------------------------------------
\newcommand{\PICK}[2]{\mbox{PICK}(#1,\  #2)}
\newcommand{\transition}[5]{\tup{#2,#3}\mapsto^{#1}\tup{#4,#5}}


\newcommand{\bigslant}[2]{{\raisebox{0em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}


\newcommand{\cts}[1]{\ensuremath{\Upsilon_#1}\xspace}
\newcommand{\sts}[1]{\ensuremath{\Theta_#1}\xspace}
\newcommand{\ncts}[1]{\cts{#1}}
\newcommand{\nsts}[1]{\sts{#1}}


\newcommand{\VT}[2]{\Upsilon^V(#1,#2)}
\newcommand{\RT}[2]{\textcolor{red}{\Upsilon(#2,#1)}}
\newcommand{\ST}[2]{\textcolor{red}{\Upsilon_S(#2,#1)}}
\newcommand{\GT}[2]{\Upsilon(#1,#2)}
%\renewcommand{\mf}[1]{{\Upsilon(\mathcal{#1})}}
\renewcommand{\mf}[1]{\Upsilon}
\newcommand{\db}{\mathit{db}}
\newcommand{\rel}[1]{\db(#1)}
\newcommand{\domdb}{\mathit{dom}}

\newcommand{\maxcalls}[2]{\ensuremath{\textsc{maxCalls}_{#2}(#1)}}



\newcommand{\ISM}[1]{\equiv_{#1}}
\newcommand{\EISM}[1]{\cong_{#1}}
\newcommand{\EMISM}[1]{\unrhd_{#1}}

\newcommand{\DUNION}{\overset{+}{\cup}}

\newcommand{\RI}{\mathfrak{I}^R}

\newcommand{\Prj}[2]{#1|_{#2}}

 \newcommand{\valueof}[1]{\ensuremath{\textsc{value}_{#1}}}
 \newcommand{\nullvalue}{\ensuremath{\chi}}
%%% END

%% Macros by Marco
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\newcommand{\realdom}{\ensuremath{\C}\xspace}
\newcommand{\scset}{\ensuremath{\mathbb{SC}}\xspace}


\newcommand{\comp}{\triangleright}
\newcommand{\bcomp}{h}

\newcommand{\UPDATE}{\mbox{UPDATE}}
\newcommand{\EXTRDIS}{\mbox{INFER\_DIS}}

\newcommand{\newskolems}{\textit{NS}}
\newcommand{\DSet}{\D}
\newcommand{\CongClosureS}{\mbox{CONGRUENCE\_CLOSURE}^S}
\newcommand{\domain}[1]{\ensuremath{\textsc{dom}(#1)}\xspace}
\newcommand{\image}[1]{\ensuremath{\textsc{im}(#1)}\xspace}

\newcommand{\embeddedfig}[2]
{
        \begin{minipage}{#2}
                \noindent
                \includegraphics[width=#2]{#1}
        \end{minipage}
}

\newcommand{\had}[1]{\domain{#1}}%{\ensuremath{\widehat{\C_{#1}}}\xspace}
\newcommand{\hd}[1]{\ensuremath{\Delta_{#1}}\xspace}
\newcommand{\rep}[2]{\ensuremath{\textsc{rep}_{#2}(#1)}}
\newcommand{\repset}[1]{\ensuremath{\textsc{rep}(#1)}}
\newcommand{\repsetc}[1]{\ensuremath{\textsc{rep}_c(#1)}}
\newcommand{\chooserep}[1]{\ensuremath{\textsc{chooseRep}(#1)}}
\newcommand{\phd}[1]{\ensuremath{\textsc{im}_{#1}}}


%\newcommand{\boxdiamond}{\ensuremath{\medbox \hspace{-.62em} \diamond}\xspace}

% \newcommand{\rewritef}[2]{\ensuremath{\textsc{rf}^{#1}_{#2}}}
% \newcommand{\rewritets}[2]{\ensuremath{\textsc{modTS}^{#1}_{#2}}}

\newcommand{\rewritefclosed}{\textsc{rf-cl}}
\newcommand{\rewritetsclosed}{\textsc{tr-cl}}
\newcommand{\rewritefinitial}{\textsc{rf-iad}}
\newcommand{\rewritetsinitial}{\textsc{tr-iad}}
\newcommand{\rewritefguarded}{\textsc{rf-gu}}
\newcommand{\rewritetsguarded}{\textsc{rf-gu}}
\newcommand{\rewritefglobal}{\textsc{rf-gl}}
\newcommand{\rewritemglobal}{\textsc{rmod-gl}}
\newcommand{\rewritetsglobal}{\textsc{tr-gl}}

\newcommand{\statename}{\textsc{sn}}

\newcommand{\someop}{\ensuremath{\circledast}\xspace}
\newcommand{\rewritemodf}{\textsc{rewriteMod}}
\newcommand{\rewritemod}[2]{\ensuremath{\rewritemodf_{#1}\left(#2\right)}}
\newcommand{\rewritequantf}{\textsc{replaceQuant}}
\newcommand{\rewritequant}[2]{\ensuremath{\rewritequantf_{#1}\left(#2\right)}}
\newcommand{\extterm}{t}
\newcommand{\somesymbol}{\circledast}



\newcommand{\globalschema}{\R}

\newcommand{\ientailment}[3]{#1\models #2#3}
\newcommand{\entailment}[4]{#1,#2\models #3#4}
%\renewcommand{\entailment}[4]{#2 \in (#3)^{#1}_{#4}}

\newcommand{\nentailment}[4]{#1,#2\not\models #3#4}
%\renewcommand{\nentailment}[4]{#2 \not\in (#3)^{#1}_{#4}}

%\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
%\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
%\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
%\DeclareSymbolFont{lasy}{U}{lasy}{m}{n}
%\DeclareMathSymbol\BlackDiamond{\mathord}{lasy}{"12}
%\DeclareSymbolFont{pxsymbolsC}{U}{pxsyc}{m}{n}
%\SetSymbolFont{pxsymbolsC}{bold}{U}{pxsyc}{bx}{n}
%\DeclareMathSymbol{\Diamondblack}{\mathrel}{pxsymbolsC}{95}
%\DeclareMathSymbol{\Squareblack}{\mathrel}{pxsymbolsC}{4}

%\newcommand{\Diamondblack}{\rotatebox[origin=c]{45}{$\Diamond$}}


%% ------------------------------------- New introduced by Babak & Alin

\newcommand{\ASINSTANCE}{\I}
\newcommand{\AINSTANCE}{I}


\newcommand{\groundexec}[2]{{\textsc{evals}_{#1}(#2)}}
\newcommand{\nrexec}[1]{{\textsc{n-exec}_{#1}\xspace}}
\newcommand{\nisexec}[1]{\textsc{nis-exec}_{#1}\xspace}
\newcommand{\skolems}[1]{{\textsc{calls}({#1})}}
\newcommand{\returns}{{\textsc{evals}}}
\newcommand{\prunings}{{\textsc{prunings}}}

\newcommand{\ERP}{{\textsc{Rcycl}}}
\newcommand{\recyclable}{{\ensuremath \mathit{RecyclableValues}}}
\newcommand{\used}{{\ensuremath \mathit{UsedValues}}}
\newcommand{\visited}{{\ensuremath \mathit{Visited}}}
\newcommand{\fresh}{{\V}}
\newcommand{\trans}{\Longrightarrow}


%%------------------------------------- Texts

\newcommand{\cstate}{\mbox{state}\xspace}
\newcommand{\sstate}{\mbox{a-state}\xspace}
\newcommand{\SINSTANCE}{\mbox{s-state}\xspace}
\newcommand{\RINSTANCE}{\mbox{c-state}\xspace}
\newcommand{\VINSTANCE}{\mbox{v-instance}\xspace}
\newcommand{\GINSTANCE}{\mbox{instance}\xspace}

\newcommand{\EISOMORPHIC}{\mbox{e-isomorphic}}

%%%%%%%%%%%%%%%%%%%%%%%%% Macros regarding the proof for Semantic Artifacts
%%\newcommand{\DOSMP}[1]{\textsc{do}\ensuremath{_\textsc{SYN}}(#1)\xspace}
\newcommand{\DOSMP}[1]{\textsc{do}_{\textsc{smp}}(#1)}
\newcommand{\mfSmp}[1]{\Upsilon_{#1,\textsc{smp}}}
\newcommand{\applySmp}[1]{\textsc{apply}_{\textsc{smp}}(#1)}
\newcommand{\Smp}{_{\textsc{smp}}}

\newcommand{\queryeq}{\ensuremath{q^{=}}\xspace}
\newcommand{\aboxeq}{\ensuremath{A_{=}}\xspace}
\newcommand{\apply}[1]{\textsc{apply}(#1)\xspace}
%\newcommand{\applySyn}[1]{\textsc{apply}\ensuremath{_\textsc{SYN}}(#1)\xspace}
% \newcommand{\conservativeTS}{conservatice}


%------------------------------------------- KAB
\newcommand{\tbox}{\T} % TBox
\newcommand{\initABox}{A_0} % Initial ABox
\newcommand{\actSet}{\Gamma} % action set
\newcommand{\action}{\gamma} % action set
\newcommand{\procSet}{\Pi} % set of process
\newcommand{\process}{\pi} % set of process


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro and personal command
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\arAns}[2][]{\textsc{ar-ans}_{#1}(#2)}

\renewcommand{\A}{A}
\renewcommand{\T}{T}
\renewcommand{\R}{R}

\newcommand{\pcts}[1]{\Theta_{#1}^\textnormal{S}}

\newcommand{\bs}[1]{\Upsilon_{#1}^{b}\xspace}
\newcommand{\cs}[1]{\Upsilon_{#1}^{c}\xspace}
\newcommand{\tsys}[1]{\Upsilon_{#1}^{t}\xspace}


\newcommand{\ctr}[1]{\Upsilon_{#1}^\textnormal{R}}
\newcommand{\vers}[2]{#1 \models_\textnormal{S} #2}
\newcommand{\itts}[1]{\Upsilon_{#1}^{\textnormal{R}}}
\newcommand{\pitts}[1]{\Theta_{#1}^{\textnormal{R}}}
\newcommand{\eitts}[1]{\Upsilon_{#1}^{\textnormal{ER}}}
\newcommand{\peitts}[1]{\Theta_{#1}^{\textnormal{ER}}}
\newcommand{\cqats}[1]{\Upsilon_{#1}^{\textnormal{CQA}}}
\newcommand{\verit}[2]{#1 \models_\textnormal{R} #2}
\newcommand{\vercqa}[2]{#1 \models_\textnormal{CQA} #2}
\newcommand{\vereit}[2]{#1 \models_\textnormal{ER} #2}

\newcommand{\skab}{S-KAB}
\newcommand{\rkab}{R-KAB}
\newcommand{\itkab}{R-KAB}
\newcommand{\ckab}{CQA-KAB}
\newcommand{\eitkab}{ER-KAB}

\newcommand{\cittransl}{\tau}

\newcommand{\qunsatf}{q^f_{\textnormal{unsat}}}
\newcommand{\qunsatn}{q^n_{\textnormal{unsat}}}
\newcommand{\lab}{\textsc{label}}
\newcommand{\viol}{\textsc{viol}}



%%%%%%%%%%%%%% GSM %%%%%%%%%%%%%%%%% Riccardo
\newcommand{\event}{\textsc{event}}
\newcommand{\stage}{\textsc{stage}}
\newcommand{\milestone}{\textsc{mlstn}}
\newcommand{\task}{\textsc{task}}
\newcommand{\lastEvent}{LastIncEventType}
\newcommand{\sentry}{\textsc{sentry}}

\newcommand{\UNTIL}{\mbox{\textbf{~U~}}}
\newcommand{\NEXT}{\mbox{\textbf{X~}}}
\newcommand{\GLOB}{\mbox{\textbf{G}}}

\newcommand{\satt}{att_s}
\newcommand{\datt}{att_d}

\newcommand{\mus}{\mathunderscore}

\newcommand{\gsm}{\ensuremath{\mathcal{G}}\xspace}



%%%%% OBDA

\newcommand{\disjoint}[2]{\ensuremath{\mathsf{disjoint}(#1,#2)}}

\newcommand{\DOMAIN}[1]{\delta(#1)}
\newcommand{\RANGE}[1]{\rho(#1)}
\newcommand{\ID}[2]{(\mathsf{id}\; #1\; #2)}
\newcommand{\Mod}[1]{\mathit{Mod}(#1)}
\newcommand{\val}[1]{\mathit{val}}
\newcommand{\ACzero}{AC^0}
\newcommand{\PerfectRef}{\ensuremath{\mathsf{PerfectRef}}\xspace}
\newcommand{\FUNCT}[1]{(\ex{funct}~#1)}
\newcommand{\atom}[3][]{\gamma_{#1}(#2,#3)}
\newcommand{\evaluate}{\mathit{eval}}
\newcommand{\Alphabet}{\Gamma}
\newcommand{\operator}{\mathsf{op}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACRO FOR SYSTEM ARCHITECTURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-------------------------------------------------
% Macro for file extension

\newcommand{\OntologyFileExtension}{owl\xspace}
\newcommand{\TempPropFileExtension}{prop\xspace}
\newcommand{\MappingFileExtension}{obgsm\xspace}

% END OF Macro for file extension
%-------------------------------------------------

%-------------------------------------------------
% Macro for Library Name

\newcommand{\ontop}{\textsc{-ontop-}\xspace}
\newcommand{\systemName}{OBGSM\xspace}
\newcommand{\marianoSystem}{\ontop}
\newcommand{\Quest}{Quest\xspace}
\newcommand{\Jena}{Apache Jena$^{\textsc{TM}}$\xspace}

% END OF Macro for Library Name
%-------------------------------------------------

%-------------------------------------------------
% Macro for temporal property

\newcommand{\AG}{\textsc{AG}}
\newcommand{\EG}{\textsc{EG}}
\newcommand{\AF}{\textsc{AF}}
\newcommand{\EF}{\textsc{EF}}
\newcommand{\AX}{\textsc{AX}}
\newcommand{\EX}{\textsc{EX}}

\newcommand{\Auntil}[2]{\textsc{A}~(#1~\textsc{until}~#2)}
\newcommand{\Euntil}[2]{\textsc{E}~(#1~\textsc{until}~#2)}

\newcommand{\andTemp}[2]{#1~\textsc{and}~#2}
\newcommand{\orTemp}[2]{#1~\textsc{or}~#2}
\newcommand{\orTempB}{~\textsc{or}~}
\newcommand{\notTemp}{\textsc{!}}
\newcommand{\implTemp}[2]{#1~\texttt{->}~#2}
\newcommand{\implTempB}{~\texttt{->}~}

\newcommand{\existsTemp}{\textsc{exists}\xspace}
\newcommand{\forallTemp}{\textsc{forall}\xspace}

\newcommand{\existsQuantification}{{\tt eQuantification}\xspace}
\newcommand{\forallQuantification}{{\tt fQuantification}\xspace}

\newcommand{\formula}{\Phi}
\newcommand{\query}{Q}
\newcommand{\guard}{{\tt{guard}}}

% END OF Macro for temporal property
%-------------------------------------------------

%-------------------------------------------------
% Macro for SPARQL

\newcommand{\variables}{{\textbf{Var}}\xspace}

%\newcommand{\varname}{{\mathbf{varname}}\xspace}
\newcommand{\triples}{{\mathbf{Triples}}\xspace}
\newcommand{\prefixDeclaration}{{\mathbf{PrefixDeclarations}}\xspace}

\newcommand{\sparql}{SPARQL 1.1\xspace}

\newcommand{\sparqlSELECT}{\textsc{Select}\xspace}

\newcommand{\sparqlWHERE}{\textsc{Where}\xspace}

\newcommand{\sparqlFROM}{\textsc{From}\xspace}

\newcommand{\sparqlDISTINCT}{\textsc{Distinct}\xspace}
\newcommand{\sparqlREDUCED}{\textsc{Reduced}\xspace}

\newcommand{\sparqlOFFSET}{\textsc{Offset}\xspace}
\newcommand{\sparqlLIMIT}{\textsc{Limit}\xspace}
\newcommand{\sparqlORDERBY}{\textsc{Order by}\xspace}

\newcommand{\sparqlOPTIONAL}{\textsc{Optional}\xspace}
\newcommand{\sparqlFILTER}{{\tt filter}\xspace}
\newcommand{\sparqlFILTEREXPRESSION}{{\tt filterExpression}\xspace}
\newcommand{\sparqlFILTERAND}{{\tt \&\&}\xspace}

\newcommand{\sparqlLT}{{\tt <}\xspace}
\newcommand{\sparqlLTE}{{\tt <=}\xspace}
\newcommand{\sparqlGT}{{\tt >}\xspace}
\newcommand{\sparqlGTE}{{\tt >=}\xspace}
\newcommand{\sparqlEQ}{{\tt =}\xspace}
\newcommand{\sparqlNEQ}{{\tt !=}\xspace}

\newcommand{\sparqlVarConst}{{\tt var\_const}\xspace}
\newcommand{\sparqlConst}{{\tt const}\xspace}
\newcommand{\sparqlString}{{\tt string}\xspace}
\newcommand{\sparqlInteger}{{\tt integer}\xspace}

\newcommand{\doubleCarret}{\mbox{\^{}\^{}}}

\newcommand{\sparqlUNION}{\textsc{Union}\xspace}

% END OF  Macro for SPARQL
%-------------------------------------------------

%-------------------------------------------------
% Macro for Mapping File

\newcommand{\prefixDeclarationMapping}{{\tt [PrefixDeclaration]}\xspace}
\newcommand{\classDeclarationMapping}{{\tt [ClassDeclaration]}\xspace}
\newcommand{\objectPropertyDeclarationMapping}{{\tt [ObjectPropertyDeclaration]}\xspace}
\newcommand{\dataPropertyDeclarationMapping}{{\tt [DataPropertyDeclaration]}\xspace}
\newcommand{\mappingDeclaration}{{\tt [MappingDeclaration]}\xspace}

\newcommand{\expression}{\psi}

\newcommand{\notGSM}{{\tt !}}
\newcommand{\andGSM}{\textsc{and}}
\newcommand{\orGSM}{\textsc{or}}

\newcommand{\getGSM}{\textbf{get}}
\newcommand{\forallGSM}{\textbf{forall}}
\newcommand{\existsGSM}{\textbf{exists}}

\newcommand{\variableGSM}{variable}
\newcommand{\constantGSM}{{\tt constant}}

\newcommand{\aopGSM}{\textbf{aop}}
\newcommand{\lopGSM}{\textbf{lop}}

\newcommand{\GSMisMSachieved}{\mathit{GSM.isMilestoneAchieved}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> submitted/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% General Math

\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}} \newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}} \newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}} \renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}} \newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}} \renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}} \newcommand{\N}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}} \renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathcal{Q}} \newcommand{\R}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}} \newcommand{\T}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}} \newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}} \newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}} \newcommand{\Z}{\mathcal{Z}}

\newcommand{\mf}{\mathfrak}

%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations

\newcommand{\setone}[2][1]{\set{#1\cld #2}}
\newcommand{\eset}{\emptyset}
%%\newcommand{\col}{\colon}
\newcommand{\ol}[1]{\overline{#1}}                % overline
\newcommand{\ul}[1]{\underline{#1}}               % underline
\newcommand{\uls}[1]{\underline{\raisebox{0pt}[0pt][0.45ex]{}#1}}

%% ul with space between text and line

\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Lra}{\Leftrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\Lora}{\Longrightarrow}
\newcommand{\lola}{\longleftarrow}
\newcommand{\Lola}{\Longleftarrow}
\newcommand{\lolra}{\longleftrightarrow}
\newcommand{\Lolra}{\Longleftrightarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\Ua}{\Uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\Da}{\Downarrow}
\newcommand{\uda}{\updownarrow}
\newcommand{\Uda}{\Updownarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%% Relations

\newcommand{\incl}{\subseteq}
\newcommand{\imp}{\rightarrow}
%%\newcommand{\deq}{\doteq}
\newcommand{\dleq}{\dot{\leq}}                   % dotted less equal

%%%%%%%%%%%%%%%%%%%%%%%%%% Spaces

\newcommand{\per}{\mbox{\bf .}}                  % period

\newcommand{\cld}{,\ldots,}                      % ,...,
\newcommand{\ld}[1]{#1 \ldots #1}                 % #1 ... #1
\newcommand{\cd}[1]{#1 \cdots #1}                 % #1 ... #1
\newcommand{\lds}[1]{\, #1 \; \ldots \; #1 \,}    % _#1_..._#1_
\newcommand{\cds}[1]{\, #1 \; \cdots \; #1 \,}    % _#1_..._#1_

%%%%%%%%%%%%%%%%%%%%%%%%%% Delimiters

\newcommand{\set}[1]{\{#1\}}                      % set
\newcommand{\Set}[1]{\left\{#1\right\}}
%%\newcommand{\bigset}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bigmid}{\Big|}
\newcommand{\card}[1]{|{#1}|}                     % cardinality of a set
\newcommand{\Card}[1]{\left| #1\right|}
\newcommand{\cards}[1]{\sharp #1}
\newcommand{\tup}[1]{\langle#1\rangle}            % tuple
\newcommand{\Tup}[1]{\left\langle #1\right\rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myi}{\emph{(i)}\xspace}
\newcommand{\myii}{\emph{(ii)}\xspace}
\newcommand{\myiii}{\emph{(iii)}\xspace}
\newcommand{\myiv}{\emph{(iv)}\xspace}
\newcommand{\myv}{\emph{(v)}\xspace}
\newcommand{\myvi}{\emph{(vi)}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%% Complexity classes

% \newcommand{\EXPTIME}{\textsc{ExpTime}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%% DL specific commands

%%%%%%%%%%%%%%%%%%%%%%%%%% Interpretation

\newcommand{\inter}[1][\I]{(\dom[#1],\Int[#1]{\cdot})}   % (dom^I,.^I)

\newcommand{\dom}[1][\I]{\Delta^{#1}}  % delta^I (domain of interpretation \I)
\newcommand{\Int}[2][\I]{#2^{#1}}      % #2^I    (interpretation function)
\newcommand{\INT}[2][\I]{(#2)^{#1}}    % (#2)^I  (interpretation function)

%%%%%%%%%%%%%%%%%%%%%%%%%% Basic Concept forming operators

\newcommand{\AND}{\sqcap}
\newcommand{\OR}{\sqcup}
\newcommand{\NOT}{\neg}
\newcommand{\ALL}[2]{\forall #1 \per #2}
\newcommand{\SOME}[2]{\exists #1 \per #2}
\newcommand{\SOMET}[1]{\exists #1}
\newcommand{\ATLEAST}[2]{(\geq #1 \, #2)}
\newcommand{\ATMOST}[2]{(\leq #1 \, #2)}
\newcommand{\EXACTLY}[2]{(= #1 \, #2)}
\newcommand{\INV}[1]{#1^{-}}

%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\vfo}{\ensuremath{v}}
\newcommand{\vso}{\ensuremath{V}}

\newcommand{\BOX}[1]{ [-] #1}
\newcommand{\DIAM}[1]{\langle - \rangle #1}

\newcommand{\ISA}{\sqsubseteq}
\newcommand{\EQU}{\equiv}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro and personal command
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\limp}{\rightarrow}
%%\newcommand{\limp}{\supset}
\newcommand{\lequiv}{\leftrightarrow}
\newcommand{\conc}{\mathord{\cdot}}

%%%%%%%%%%% Mu-Calculus Interpretation: \mf{A}, \V

\newcommand{\MOD}[1]{(#1)^\mf{A}}
\newcommand{\Moda}[1]{#1_{\V}^\mf{A}}     % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.
\newcommand{\Modax}[2]{#1_{\V #2}^\mf{A}} % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and modif. assign. fun.
%\newcommand{\MODA}[1]{(#1)_{\V}^\mf{A}}   % (argument)_{\V}^\mf{A} % Giuseppe
%                                        % interp. and assign. fun.
%\newcommand{\MODAX}[2]{(#1)_{\V #2}^\mf{A}} % (argument)_{\V.}^\mf{A} % Giuseppe
%                                        % interp. and
%                                        % modif. assign. fun.

\newcommand{\MODA}[1]{(#1)_{\vfo,\vso}^\mf{A}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.

\newcommand{\MODAfirst}[1]{(#1)_{\vfo}^\mf{A}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.


\newcommand{\MODAX}[2]{(#1)_{\vfo #2,\vso}^\mf{A}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.

\newcommand{\MODAZ}[2]{(#1)_{\vfo,\vso #2}^\mf{A}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.




\newcommand{\MODATX}[3]{(#1)^{#2}_{#3}}

\newcommand{\Modat}[2]{#1_{\V}^{#2}}     % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.
\newcommand{\MODAT}[2]{(#1)_{\V}^{#2}}   % (argument)_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}

 \newcommand{\dllite}{\textit{DL-Lite}\xspace}
 \newcommand{\dllitef}{\textit{DL-Lite}\ensuremath{_{\mathcal{F}}}\xspace}
 \newcommand{\dlliter}{\textit{DL-Lite}\ensuremath{_{\mathcal{R}}}\xspace}
 \newcommand{\dllitea}{\textit{DL-Lite}\ensuremath{_{\mathcal{A}}}\xspace}
\newcommand{\dllitenouna}{\textit{DL-Lite}\ensuremath{_\textsc{nu}}\xspace}


\newcommand{\cert}[1]{\mathit{cert}(#1)}
\newcommand{\ans}[2][]{\mathit{ans}_{#1}(#2)}
\newcommand{\rew}[1]{\mathit{rew}(#1)}
\newcommand{\goto}[1][\mf{A}]{\mathrel{\Ra_{#1}}}

\newcommand{\conj}{\mathit{conj}}

\newcommand{\homom}[4][\C]{#3 \mathrel{\ra^{#1}_{#2}} #4}
\newcommand{\map}[2]{#1 \rightsquigarrow #2}
\newcommand{\carule}[2]{#1 \mapsto #2}

% \renewcommand{\A}{A}
% \renewcommand{\T}{T}
% \renewcommand{\R}{R}
%%\renewcommand{\C}{C} %%%GGG altrimenti si confonde con i concetti

\newcommand{\Amax}{\A_{\mathit{max}}}

\newcommand{\ex}[1]{\mathsf{#1}}
\newcommand{\actex}[1]{\mathsf{#1}}


\newcommand{\bsy}[1]{\boldsymbol{#1}}
\newcommand{\brho}{\bsy{\rho}}
\newcommand{\bpi}{\bsy{\pi}}



%% For KR 2012
\newcommand{\funct}[1]{(\ex{funct}~#1)}
\newcommand{\idconstr}[2]{(\ex{id}~#1~#2)}
\newcommand{\adom}[1]{\textsc{adom}(#1)}
\newcommand{\idom}[1]{\textsc{idom}(#1)}

\newcommand{\eq}[2]{#1 = #2}
\newcommand{\Eq}[1]{\textsc{eq}(#1)}
\newcommand{\DO}[1]{\textsc{do}(#1)}

\newcommand{\Ans}[2][]{\textsc{ans}_{#1}(#2)}
\renewcommand{\=}{\hspace{-0.08cm}=\hspace{-0.08cm}}

%\newcommand{\norm}[1]{#1 \withinit \hspace{-0.15cm} \_}
%\newcommand{\norm}[1]{#1 \hspace{-0.05 cm} \scriptsize{\rotatebox[origin=c]{180}{$\textcypr{\Cte}$}}}
\newcommand{\norm}[1]{#1^*}
\newcommand{\fnorm}{norm}
\newcommand{\UNA}{\textsc{\tiny{UNA}}}

%\newcommand{\norm}[1]{\lceil #1 \rceil}

\newcommand{\Tuna}{T^{\textsc{una}}}
\newcommand{\Tnouna}{T^{\st{\textsc{una}}}}

\newcommand{\fabox}{\mathit{abox}}
\newcommand{\abox}{\mathit{abox}}
%%\renewcommand{\do}{do}

\newcommand{\compactTS}{\mathcal{T}_s^c}

\newcommand{\homeq}{\stackrel{h}{=}}


\newcommand{\PTIME}{\textsc{PTime}\xspace}
\newcommand{\EXPTIME}{\textsc{ExpTime}\xspace}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

